Argus: A Fully Transparent Incentive System for Anti-Piracy Campaigns (Extended Version)

Anti-piracy is fundamentally a procedure that relies on collecting data from the open anonymous population, so how to incentivize credible reporting is a question at the center of the problem. Industrial alliances and companies are running anti-piracy incentive campaigns, but their effectiveness is publicly questioned due to the lack of transparency. We believe that full transparency of a campaign is necessary to truly incentivize people. It means that every role, e.g., content owner, licensee of the content, or every person in the open population, can understand the mechanism and be assured about its execution without trusting any single role. We see this as a distributed system problem. In this paper, we present Argus, a fully transparent incentive system for anti-piracy campaigns. The groundwork of Argus is to formulate the objectives for fully transparent incentive mechanisms, which securely and comprehensively consolidate the different interests of all roles. These objectives form the core of the Argus design, highlighted by our innovations about a Sybil-proof incentive function, a commit-and-reveal scheme, and an oblivious transfer scheme. In the implementation, we overcome a set of unavoidable obstacles to ensure security despite full transparency. Moreover, we effectively optimize several cryptographic operations so that the cost for a piracy reporting is reduced to an equivalent cost of sending about 14 ETH-transfer transactions to run on the public Ethereum network, which would otherwise correspond to thousands of transactions. With the security and practicality of Argus, we hope real-world anti-piracy campaigns will be truly effective by shifting to a fully transparent incentive mechanism.

==> Argus SRDS Full/arch.tex <==
 \subsection{Implementation details} \label{sec:imple}

Argus' implementation\footnote{We will publish the source code of our implementation in the near future.} spans over three technology areas: watermarking (embedding, detection), cryptography (OT, PIR, etc.), contract (contract code and client script). For watermarking, we integrate existing algorithms of three data types (i.e., image, audio, software) currently. Other data types could be added in the future. For cryptography and contract, we implement and optimize the designs using the insights and ideas described in Appendix \ref{sec:contract} and Appendix \ref{sec:crypto}. 
%In addition, we will introduce further detailed optimization of protocols and contracts in Section \ref{sec:construct}.

Instantiation is about the setup of parameters and algorithms described in Appendix \ref{sec:bigpic}, which directly impacts the security analysis of Argus in Section \ref{sec:eval}. We will provide the parameter and the algorithm utilized in this work especially in Appendix \ref{sec:crypto}.

\subsubsection{Digital Watermarking}\label{sec:wmimple}
We leverage Spread Spectrum (SS) based watermark for the images \cite{image} and audio \cite{audio}; Control flow graph (CFG) watermark for the software \cite{software}. As described in Section \ref{sec:model}, watermark-related attack \cite{sensitivity, bibd} is not considered in this work. Corresponding countermeasures are orthogonal to this work and thus can be further applied to increase the security of our system. The setup of watermarking parameters are listed in Table \ref{tab:wm}. In addition, we also list the performance and effect of watermark embedding/detection. 

\vspace{5pt}
\noindent {\bf Further Optimization.} Intuitively, the watermark embedding may take considerable time for the owner to initiate if the $N$ is large with an overhead of $O(N*M)$. In fact, this overhead can be mitigated with segment-and-watermark technology \cite{ot2,ot1}: to split the data into $L$ multiple segments and randomly embed each segment with an alternative watermark from $\set{w_1,w_2}$. Then, by randomly combining the segments, it is easy to obtain $2^L$ versions of watermarked data. The whole process only costs twice of watermark embedding time. In addition, since the watermark embedding time is offline and setup only once, the overhead of this part is totally acceptable.

\begin{table}[thbp]
\centering
\footnotesize
% \vspace{-10pt}
\caption{The details of watermarking schemes}
\vspace{-5pt}
\setlength{\tabcolsep}{3pt}
 \renewcommand{\arraystretch}{1.1}
 \begin{threeparttable}
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{Types}   & \multirow{2}{*}{Configuration \& Implementation}                                                                            & \multicolumn{2}{c|}{Latency} \\ \cline{3-4} 
                         &                                                                                                                         & $E_w$     & $D_w$    \\ \hline
Image  \cite{image}      & \begin{tabular}[c]{@{}c@{}}512$\times$512 image ($\sim 256$ KB), \\ 128 segments, 40dB PSNR, DCT algorithm\end{tabular} & 3.0 s         & 2.2 s        \\ \hline
Audio \cite{audio}       & \begin{tabular}[c]{@{}c@{}}44100 Hz, 1 second wav ($\sim$ 344 KB), \\ MCLT-based watermarking algorithm\end{tabular}    & 4.8 s         & 3.1 s        \\ \hline
Software \cite{software} & \begin{tabular}[c]{@{}c@{}}Geth binary ($\sim$ 20 MB), \\ Obfuscated CFG with 128-bit watermark\end{tabular}            & 1.7 s         & 2.5 s        \\ \hline
\end{tabular}
% \begin{tablenotes}
%\item[*] $E_w$ and $D_w$ represent watermark embedding and detection, respectively (details in Section \ref{sec:holistic})
% \end{tablenotes}
\end{threeparttable} \label{tab:wm}
\vspace{-10pt}
\end{table} 

\subsubsection{Contract} \label{sec:contract}
For the ledger, we leverage one of the most popular and commercially successful platforms, Ethereum \cite{ethereum}, to deploy and test our contract. Accordingly, we implement Argus contract with $\sim 2,400$ lines of code in Solidity $^\land0.4.23$ \cite{solidity}. It is developed in Truffle $4.1.14$ \cite{truffle} and deployed to a blockchain of $10$ nodes running 
% Ganache CLI v6.8.0-istanbul.0 (ganache-core: 2.9.0-istanbul.0) \cite{ganache}
Geth istanbul version v$1.9.3$ \cite{geth} to emulate the public Ethereum (similar to Ropsten Testnet\cite{testnet}).   

\vspace{5pt}
\noindent {\bf Further Optimization.} We further optimize $\mathsf{VerifyReport}$, which is one of the most expensive functions of contract $\mathcal{C}$. We apply a caching strategy, of which the main idea is simple: every time every informer submits a path of Merkle tree to the contract for verification, which not only introduces considerable on-chain bandwidth overhead but also on-chain hash operations. To mitigate the overhead, we let the contract memorize the path submitted by previous informers. For the incoming informers, only the non-overlapped part of the path is submitted and checked by the contract $\mathcal{C}$. Therefore, given the temporal locality of piracy distribution, most of the paths submitted by adjacent informers are overlapped and can be omitted. Our results show that the caching strategy can reduce 31\% of the gas consumption.

%Given that a typical blockchain (Bitcoin, Ethereum) can only handle $\sim$ 10 transactions per second and the process of OT involves multiple interactions/transactions, we leverage the state channel technology to reduce the overhead \cite{plasma,arbitrum}. Ideally, with the state channel, transactions are only sent to the chain at the start/end of data deliveries. However, to support the report submission process, corresponding $\{H(ID_i)\}$ should be public, which is considerably large per deal. Thus, we construct a Merkle tree data structure to store $\{H(ID_i)\}$ offchain, while leveraging the blockchain's immutability, as shown in Figure \ref{fig:mt}. As soon as a new trade [* what is a trade?-shuo *] occurs, the Merkle tree is updated, and only its root is sent to the contract. And the rest of the Merkle tree can be kept offchain (e.g. in owner's bulletin board). 

%[* Has Xian made a pass for this section -Shuo * ]
%Since a reporter needs to prove his/her possession of a valid $ID_i$, the list of $\{ID_i\}$ should be obtained first. However, direct querying the bulletin board exact $ID_i$ may leak the value of $ID_i$ to the owner. To mitigate the leakage, we embed additional bits in the ID called ``Trade-ID'', namely Watermarked ID is a catenation of a secret ID and a Trade-ID. once the whistleblower detects the Watermark ID, he or she should query the subtree corresponding to the Trade-ID and obtains the entire subtree. With the subtree, the whistleblower can then generate the two proofs:
%\begin{enumerate}
%    \item The detected secret ID is in a certain path of the subtree.
%    \item There is a path traversing from the root of subtree to the root of the whole Merkle tree. 
%\end{enumerate}
%
%As illustrated in Figure \ref{fig:mt}, the first proof is required to be zero-knowledge to prevent lekage to owner while the second can be implemented using Merkle tree proof for better prover performance. Note that we catenate ${H(ID_i)}$ with index $i$ to facilitate the appealling process of users. As addressed in Section \ref{sec:zkw}, the whistleblower should send the proof along with an encryption of the answer to the contract. And the user can appeal to the contract that the decrypted answer is invalid via BLS signature. 
%By contrast, for the structure in Figure \ref{fig:mt}, the whistleblower should send the encryption of ${H(ID_i)}||i$ to the contract and the user appeals as follows:
%\begin{enumerate}
%    \item The user decodes $H(ID'_i)$ and the index $i$ from the decryption of ${H(ID'_i)}||i$ and proves the correctness of the decoding with BLS signature. 
%    \item The user proves that $i$-th leaf ${H(ID_i)}||i$ in the subtree conflicts with decoded $H(ID'_i)$ or conflicts with $PK_0$ during asymmetric watermarking. 
%    \item If the ${H(ID'_i)}||i$ is incorrect in index $i$ but exists in subtree, the owner loses in the appeal and the licensee is innocent. 
%\end{enumerate}
% \begin{figure}[thbp]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figs/mt.pdf}
%     \caption{The Merkle Tree for $H(ID)$ }
%     \label{fig:mt}
% \end{figure}
\subsubsection{Cryptography} \label{sec:crypto}
For cryptographic modules, we customize our OT protocol\cite{np} based on libOTe \cite{libote}, which is one of the state-of-the-art implementations of OT atop the Miracle Library \cite{miracle}. We set $N$ as $10,000$ to achieve an sufficient security strength. For the symmetric encryption, asymmetric encryption (e.g. for generating signature) and hash algorithms, we set $\lambda$ as $128$ and leverage AES, ECCSA, SHA-256 implemented in the Miracle library, respectively. In addition, in order to be compatible with Web3 in Ethereum \cite{web3}, we adapt the ECC in Miracle to be based on BN-$254$ curve \cite{bn254}. And with the SHA-256 algorithm, we implement the Merkle tree algorithm. For multi-period commitment scheme, we set $K$ as $1000$ and the period of report collection as $180$ days, which means that an informer's report is confirmed at most in $180*24/1000=4.32$ hours.  In addition, we leverage state-of-the-art PIR, XPIR, which is highly optimized by using Ring-LWE \cite{xpir}.

\vspace{5pt}
\noindent {\bf Further Optimization.} We optimize $\mathsf{Initiate}$ to reduce storage overhead for the owner. For a straightforward design, we can have the Merkle tree as a three-layered structure: the first layer (near the tree top $rt$) has $O(M)$ leaves which corresponds to licensees; the second layer, of which the tree top is the leave of the first layer, has $O(M*N)$ leaves which corresponds to $N$ versions of OT data; and similarly, the third has $O(M*N*K)$ corresponding to the timestamps. For the owner, only the leaves of the second layers are stored locally and provided with a storage overhead of $O(N)$ per licensee. With these leaves, the informers can generate the entire Merkle tree according to the timestamp and these leaves. 
% Furthermore, the owner can further store a treetop of Merke tree $rt$ (e.g. $k=3$ levels), which can reduce informers' generation time of Merkle tree $2^k$ times.

%We generate the binary for ZK prover and the contract for ZK verifier using Zokrates \cite{zokrates}. For the PIR part, we adopt the state-of-the-art implementation of computational PIR called XPIR \cite{xpir}, which is demonstrated of high scalability. There are also miscellaneous parts which utilize cryptographic operations, such as signing, state channel, BLS signature, Merkle tree, etc. For these parts, blockchain compatible algorithms are leveraged referring to the implementation of Web3 \cite{web3}.

We also optimize the off-chain bandwidth overhead incurred in $\mathsf{TransferData}$. For OT protocol where $N=10,000$, compared to the intended data, $10,000$ times of data size are transferred between the owner and the licensee (Figure \ref{fig:ot}). In addition, the performance overhead of asymmetric encryption/decryption also burdens the owner/licensee. Therefore, we adapt the process of OT to mitigate the overhead of asymmetric encryption and introduce Private Information Retrieval~(PIR) \cite{xpir} to mitigate the bandwidth overhead: data are first encrypted with symmetric encryption (e.g. AES) and only keys are transferred via OT. The encrypted data are then downloaded by the licensee with PIR protocol in an offline style. With these optimizations, the overhead of bandwidth and performance can be largely reduced, which is shown in Section \ref{sec:eval}.
%
%\squishlisttwotwo
%    \item The owner encrypts $N$ copies of data using symmetric encryption (e.g. AES) with $N$ secret keys $\{PrivK_i\}$, which is denoted as $\{Enc_{PrivK_i}(D_i)\}$
%    \item The licensee gets $K_j$ from $\{PrivK_i\}$ via $1$-out-of-$N$ OT protocol.
%    \item The licensee gets encrypted $Enc_{PrivK_j}(D_j)$ from $\{Enc_{PrivK_i}(D_i)\}$ via PIR protocol.
%    \item The licensee decrypts $Enc_{PrivK_j}(D_j)$ with $PrivK_j$.
%\squishlisttwotwoend
%For the bandwidth overhead, the above scheme can achieve the same security with a bandwidth consumption of $\Psi(|D|+N*|PrivK|)$. Given that $|D|\gg |PrivK|$, the bandwidth overhead is $\Psi(|D|)$ which approximates the original data size. For the performance overhead, the symmetric encryption phase can be conducted offline and thus can be omitted. The performance of PIR is highly optimized by using Ring-LWE \cite{xpir}. The overhead of decrypting $Enc_{PrivK_j}(D_j)$ is negligible compared to the network latency. The overhead of bandwidth and performance is evaluated in Section \ref{sec:eval}.


==> Argus SRDS Full/eval.tex <==
\section{Security Analysis and Performance Evaluation}\label{sec:eval}
In this section, we first analyze the security of Argus then describe the experimental setup for the performance evaluation. The evaluation results include the performance measurements and the cost of Argus transactions.

\subsection{Security Analysis} \label{sec:analysis}

\begin{table}[]
\centering
\footnotesize
\caption{Interests/threats of participants in argus}
\setlength{\tabcolsep}{3pt}
 \renewcommand{\arraystretch}{1.1}
\begin{tabular}{|c|c|c|}
\hline
Participants & Interest if honest                                                                                         & Threat if malicious                                                             \\ \hline
Owner        & \begin{tabular}[c]{@{}c@{}}To discover infringers and\\ tally the number of copies\end{tabular} & \begin{tabular}[c]{@{}c@{}}To falsely accuse \\ innocent licensees\end{tabular}       \\ \hline
Licensee     & \begin{tabular}[c]{@{}c@{}}To win in an appeal \\ because of innocence\end{tabular}  &  \begin{tabular}[c]{@{}c@{}}To appeal despite \\ the guilt\end{tabular}      \\ \hline
Informer     & \begin{tabular}[c]{@{}c@{}} To submit a honest \\ report once  \end{tabular}   & \begin{tabular}[c]{@{}c@{}}To submit a fake report, \\ steal a report  or submit a \\ valid report multiple times. \end{tabular} \\ \hline
\end{tabular}
\label{tab:interest}
\vspace{-15pt}
\end{table}

The detailed security analysis is given in Appendix \ref{sec:proof}. Without loss of generality, we only present an analysis which considers a game of five participants $\mathsf{Game}^{Argus}_{O, L_1, {L_2},I_1, {I_2}}$, where $O, L_1, {L_2},I_1, {I_2}$, representing the Owner, one Licensee, another Licensee, one Informer and another Informer, respectively. Their interests if honest and their threats if malicious are summarized in Table
\ref{tab:interest}. Based on $\mathsf{Game}^{Argus}_{O, L_1, {L_2},I_1, {I_2}}$, we can easily extend our security analysis to scenarios with multiple owners, informers and licensees. Since $L_1$ and $I_1$ are identical to $L_2$ and ${I_2}$ respectively, to demonstrate the security of Argus, we enumerate all cases that $O, L_1, I_1$ is individually honest (i.e. following the protocol) while other four participants may collude. For each case, we find that the interest of the honest participant will not be affected. In other words, we conclude that {\em if a participant (i.e. owner, licensee or informer) has no fault, the interest of this participant will not be hurt even when others collude.} 

\subsection{Performance Evaluation}
\noindent{\bf Experimental Setup.} Our testbed consists of relatively low-end Azure Virtual Machines (D2s\_v3, 2 vCPUs, 8GB RAM, Linux) for the nodes of owner, licensees, informers and blockchain nodes. For blockchain nodes, we adopt the default PoW algorithm (ie. Ethash \cite{ethereum}) and parameters (block interval, block Gaslimit, etc.) of current Ethereum (date: 2021-04-05) to simulate the public blockchain. The average block interval of Ethereum is set to 12 seconds. The bandwidth of uploading and downloading is tested as around $50$ MB/s. To guarantee a sufficient OT security and a short confirmation of reports, we by default set the OT versions (i.e., N) in Section \ref{sec:detect} as 10,000 while the number of periods (i.e., K) in Section \ref{sec:zkw} as 1000. In other words, the probability to accuse an innocent licensee is $\frac{1}{10000}$ while the report confirmation time during a 180-day period is 4.3 hours. The implementation details of Argus is described in Appendix \ref{sec:bigpic} and Appendix \ref{sec:imple}. 

% \begin{table}[]
% \small
% \caption{Parameters of experimental setup}
% \centering
% \begin{tabular}{|c|c|c|c|}
% \hline
% Parameters & Block Interval & GasPrice & Ethereum Price   \\ \hline
% Values     & $\sim12$ s           & $\sim$$12$ Gwei   & $\sim$\$$230$                       \\ \hline
% \end{tabular}
% \label{tab:config}
%  \vspace{-5pt}
% \end{table}
% \footnote{Retrieval date at 2019\-10\-30 from \cite{coinmarket}}  

%\begin{table}[]
%\caption{Parameters of Experimental Setup}
%\begin{tabular}{|l|l|}
%\hline
%Parameters         & Values \\ \hline
%Block interval     & 12 s   \\ \hline
%GasPrice           & 4G wei \\ \hline
%Ethereum Price     & 200 \$ \\ \hline
%\#Blockchain nodes & 10     \\ \hline
%\end{tabular}
%\label{tab:config}
%\end{table}

%The corsortium blockchain (Quarum) are also simulated with similar settings. The details of algorithm and optimization are introduced in last Section.





%Standard D2s v3 (2 vcpus, 8 GB memory) US$71.42        linux2
%Standard NC24r (24 vcpus, 224 GB memory) US$3,548.88   dnnwatermark
%Standard D32s v3 (32 vcpus, 128 GB memory) US$1,142.78 linux1
%Standard D16s v3 (16 vcpus, 64 GB memory) US$571.39    linux3
\vspace{5pt}
\noindent {\bf  Evaluation Results.} We evaluate Argus system from various perspectives of practicality, such as the throughput of system, client latency, gas cost on Ethereum, etc. All protocols of Argus are tested end-to-end. We also give the comparison between Argus and previous work from aforementioned perspectives. Due to the page limit, we only present evaluation results of $\mathsf{Initiate}$, $\mathsf{ShareData}$, $\mathsf{ReportPiracy}$ and $\mathsf{Appeal}$, which are the most resource-consuming protocols (details in Appendix \ref{sec:view}). In other words, these four protocols can introduce considerable overhead in throughput, latency, storage and cost to impede the Argus's adoption in practice. For an intuitive understanding of the gas cost in Ethereum, we represent the gas cost in the number of sending simplest transactions\footnote{Ethereum's simplest transaction only transfers ether and costs 21,000 gas.}.

We first evaluate $\mathsf{Initiate}$, which is the setup phase of Argus. The main elements of $\mathsf{Initiate}$ is to generate an Merkle tree and to deploy the contract. For every licensee, there is a time complexity of $O(N*K)$ for the owner to generate the Merkle tree, which needs about $10$ minutes. This process is totally offline and can be parallelized and accelerated with high-end machines. Deploying the contract costs about $5.2\times 10^6$ gas, which equals to the cost of sending $\sim$248 simplest Ethereum transactions. In addition, we also evaluate the off-chain storage cost for Argus, which is about 960 KB per licensee, which has a space complexity of $O(N)$. 

\begin{table*}[tbhp]
\footnotesize
 \centering
 \caption{High-level comparison between state-of-the-art work and Argus}
 \vspace{-5pt}
 \setlength{\tabcolsep}{3pt}
 \renewcommand{\arraystretch}{1.1}
  \begin{threeparttable}
 \begin{tabular}{llcccccccc}
 \hline
 \multicolumn{1}{c}{Desired properties}            & \multicolumn{1}{c}{Details}           & BSA \cite{bsa} & Custos \cite{custos} & AWM \cite{ot3} & ZKP \cite{zerocash} & Hydra \cite{hydra} & Arbitrum \cite{arbitrum} & This work        \\ \hline
Trusted payments & Full transparency         & $\times$\tnote{*}             & $\surd$                  & N/A\tnote{**}                         & $\surd$                    & $\surd$               & $\surd$                      & $\surd$          \\
   Better payments                   & Timely/guaranteed payout   & $\times$          & $\surd$                  & N/A                         & $\surd$                    & $\times$                & $\times$                      & $\surd$          \\  
   Identifying infringers                  & Strong accusation  & $\surd$         & $\times$                  & $\surd$                     & N/A                & N/A                 & N/A                      & $\surd$     \\ 

 \multirow{2}{*}{Assessing severity}  
 & Sybil-proofness              & $\surd$               & $\times$                      & N/A                         & N/A                    & N/A                & $\surd$              & $\surd$          \\  
 & Information-hiding               & $\surd$               & $\times$                      & N/A                         & $\surd$                    & $\surd$        & $\surd$                       & $\surd$          \\
                                 
 Scalability                     & High throughput       & $\surd$           & $\times$                  & $\times$                     & $\times$                & $\surd$            & $\surd$                  & $\surd$ \\ \hline
 \end{tabular}
%  \label{tab:compare}
 \begin{tablenotes}
 \item[*] Symbols of ``$\surd$'' and ``$\times$'' denote corresponding property is ``achievable'' and ``hard to achieve'', respectively. 
 \item[**] Properties are marked as ``not applicable (N/A)'' if corresponding work is not designed for these properties.
 \end{tablenotes}
 \end{threeparttable}\label{tab:compare}
 \vspace{-15pt}
 \end{table*}
 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\textwidth]{figs/ot.pdf}
    \vspace{-15pt}
    \caption{The performance of OT and PIR: (a) OT Latency (b) PIR Latency (c) PIR Latency for different data}
    \label{fig:otpir}
    \vspace{-15pt}
\end{figure}

We evaluate the latency/bandwidth in data sharing. $\mathsf{ShareData}$ includes two phases, OT (Section \ref{sec:detect}) and PIR (Appendix \ref{sec:imple}). While the PIR phase can be done offline, the OT phase can directly affect the throughput of the Argus system especially when there are a number of clients (licensees) concurrently communicating with the server (owner):
\squishlistoneone
 \item For the OT phase, the evaluation result is shown in Figure \ref{fig:otpir} (a). It takes about $141$ ms for the server to complete the phase. Therefore, a throughput of $7.1$ OT requests per second per machine can be served. With a stronger server (Azure D32s\_v3, $32$ cores, $128$GB RAM), the throughput can be further improved to $82.6$ per second. Note that, the throughput can be linearly scaled up by increasing the number of machines.
 \item For the PIR phase, we list the latency of client/server in Figure \ref{fig:otpir} (b) and Figure \ref{fig:otpir} (c). As shown in Figure \ref{fig:otpir} (b), the PIR latency is proportional to the data size, which corresponds to a bandwidth of $206$ Kbps and $476$ Kbps for the client and server, respectively. And with Figure \ref{fig:otpir} (b), we have the PIR latency for data types in Table \ref{tab:wm} (Appendix \ref{sec:wmimple}), which is shown in Figure \ref{fig:otpir} (c). Without PIR, the direct downloading time of the 10,000 copies for the licensee would be 51 s, 67 s and 3800 s, respectively. Similar to the OT phase, the latency and bandwidth of PIR phase can also be linearly and considerably improved with more and higher-performance (i.e. faster core and larger RAM) machines. Since PIR can be offline after the OT phase, the bandwidth of Argus system is determined by the OT phase.
\squishlistoneoneend

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%\begin{table}[]
%\footnotesize
% \setlength{\tabcolsep}{1.3pt}
% \renewcommand{\arraystretch}{1.1}
% \centering
% \caption{Comparison of performance and gas cost between previous work and Argus}
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%Protocols                     & Main elements                                                                   & Latency                                                                 & Gas                                                                                           & Fee                          \\ \hline
%Initiate                      & \begin{tabular}[c]{@{}c@{}}GenerateMerkleTree\\and DeployContract\end{tabular} & \begin{tabular}[c]{@{}c@{}}605 s \\ per licensee\end{tabular}      & $5.2\times 10^6$                                                                             & \multicolumn{1}{c|}{\$ 14.5}  \\ \hline
%ShareData                     & OT                                                                           & \begin{tabular}[c]{@{}c@{}}Client: 254 ms\\ Server: 141 ms\end{tabular} & N.A.                                                                                          & \multicolumn{1}{c|}{N.A.}    \\ \hline
%\multirow{2}{*}{ReportPiracy} & ZKP \cite{zkbounty,zkpcommit}                                                          & 45 s                                                                   & $4.6\times 10^5$                                                                             & \multicolumn{1}{c|}{\$ 1.28} \\ \cline{2-5} 
%                              & Multi-period                                                                 & \begin{tabular}[c]{@{}c@{}}Commit: 79 ms\\ Reveal: 295 ms\end{tabular}  & \begin{tabular}[c]{@{}c@{}} $8.0\times 10^4$\\  $2.0\times 10^5$\end{tabular} & \multicolumn{1}{c|}{\$ 0.78}  \\ \hline
%\multirow{2}{*}{Appeal}       & O(N) \cite{ot1,ot2}                                                          & 85 s (esti.)                                                            & $2.4\times 10^8$ (esti.)                                                                     & \multicolumn{1}{c|}{\$ 442}   \\ \cline{2-5} 
%                              & O(1)-Appeal                                                                  & 278 ms                                                                  & $2.3\times 10^5$                                                                             & \multicolumn{1}{c|}{\$ 0.62}  \\ \hline
%\end{tabular}
% \vspace{-5pt}
% \label{tab:perfcompare}
%\end{table}

% \begin{table}[]
% \caption{Evaluating $\mathsf{ShareData}$, $\mathsf{ReportPiracy}$ and $\mathsf{Appeal}$}
% \centering
%  \setlength{\tabcolsep}{5pt}
%  \renewcommand{\arraystretch}{1.0}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{} & \multicolumn{2}{c|}{ShareData} & \multicolumn{2}{c|}{ReportPiracy} & Appeal    \\ \cline{2-6} 
%                   & Client         & Server        & Commit         & Reveal           &           \\ \hline
% Latency (ms)      & 254            & 252           & 79             & 295              & 278     \\ \hline
% Gas               & N.A.           & N.A.          & 72188          & 255629           & 256359 \\ \hline
% \end{tabular}
% \label{tab:perf}
% \end{table}

%\begin{table}[]
%\centering
%\small
%\caption {The performance of PIR}
%\setlength{\tabcolsep}{4.5pt}
% \renewcommand{\arraystretch}{1.0}
%\begin{tabular}{|c|c|c|c|}
%\hline
%PIR Latency (s)                   & Image       & Audio       & Software    \\ \hline
%Client Latency($\sim$ 206 Kbps) & 9.9 s & 13.3 s & 12 min 55s \\ \hline
%Server Latency($\sim$ 476 Kbps) & 4.3 s & 5.8 s & 5 min 36 s \\ \hline
%\end{tabular}
%\label{tab:pir}
% \vspace{-15pt}
%\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\textwidth]{figs/zkp.pdf}
    \vspace{-20pt}
    \caption{Comparison of previous work (i.e. ZKP \cite{zkbounty,zkpcommit}  ) and multi-period commitment scheme: (a) Latency (b) Gas Cost}
    \label{fig:zkp}
    \vspace{-10pt}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\textwidth]{figs/appeal.pdf}
    \vspace{-20pt}
    \caption{Comparison of previous work (i.e. O(N)-Appeal \cite{ot1,ot2}  ) and O(1)-Appeal: (a) Latency (b) Gas Cost}
    \label{fig:appeal}
    \vspace{-15pt}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{figs/sensitivity.pdf}
    \vspace{-5pt}
    \caption{Sensitivity analysis of \#OT versions: (a) Latency (b) Gas Cost}
    \label{fig:sensitivity}
    \vspace{-20pt}
\end{figure}

$\mathsf{ReportPiracy}$ includes the commit phase and the reveal phase (Section \ref{sec:zkw}). The evaluation results of $\mathsf{ReportPiracy}$ are shown in Figure \ref{fig:zkp}. The latency in Figure \ref{fig:zkp} (a) denotes the time which is spent by Informer's machine to submit a transaction to Argus contract until the transaction is executed by blockchain nodes. In other words, the consensus time is excluded in the latency result. The latency of commit and reveal are negligible compared to the block time of Ethereum. 

The on-chain cost of our multi-period scheme is also negligible. As shown in Figure \ref{fig:zkp} (b), the gas cost for commit and reveal are about $8*10^4$ and $2*10^5$, which equals to $\sim$3 and $\sim$11 simplest Ethereum transactions, respectively. In other words, a total cost equivalent to sending 14 simplest transactions is required for an informer to report a piracy in our system. From the gas consumption, given that the maximum gas limit of every Ethereum block is around $12,000,000$, we can conclude that the Transactions Per Second (tps) for ReportPiracy is about $12*10^6/(2.0*10^5*12) \approx 5.0$, which is 11\% of the theoretically maximum Ethereum throughput\footnote{The maximum tps of Ethereum is about $47.6$ when the block only contains simplest Ethereum transactions. By contrast, the average tps of Ethereum is $15.0$ currently (2021-04-05).} (commit and reveal occur in different blocks and thus only the more expensive reveal is considered). We also compare our multi-period scheme with ZKP scheme \cite{zkbounty,zkpcommit}. Compared to ZKP scheme, our scheme can reduce the informer client latency by $99.3$\% and the gas cost by $39$\%.


As in Figure \ref{fig:appeal}, we also evaluate $\mathsf{Appeal}$ (Section \ref{sec:detect}) and get similar results as $\mathsf{ReportPiracy}$: a tps of $4.3$ is achieved given the gas consumption of $\mathsf{Appeal}$ ($\sim 2*10^5$, i.e., the cost of $\sim$11 simplest Ethereum transactions). The appeal protocol proposed by previous work \cite{ot1,ot2} (denoted as ``$O(N)$-Appeal'') introduces unacceptable on-chain operations and exceeds the maximum gas-limit of an Ethereum block. Thus, we cannot evaluate corresponding latency and gas consumption in an end-to-end style. Instead, we estimate them using the number of on-chain operations. Results show that $O(1)$-appeal can significantly reduce the client latency and the gas cost: compared to previous appeal scheme, the informer client latency can be reduced by $99.7$\% and the gas cost by a factor of $960$X, respectively.


As shown in Figure \ref{fig:sensitivity}, we also investigate the impact of choosing different numbers of OT versions (i.e. $N$), from $10$ to $10,000$. On one hand, as addressed in Section \ref{sec:detect}, the value of $\frac{1}{N}$ determines the probability $\phi$ of false accusation; On the other hand, the increase of $N$ has a negative impact on the performance, gas cost and storage overhead of Argus system (Appendix \ref{sec:crypto}). We can see that the increase of OT affects the OT latency of owner significantly (Figure \ref{fig:sensitivity} (a)) while the gas cost increases logarithmically (Figure \ref{fig:sensitivity} (b)) since we use Merkle tree structure in our design (details in Appendix \ref{sec:view})\footnote{We omit the commit operation of informer in Figure \ref {fig:sensitivity} since the latency and gas cost of commit is unrelated to the value of $N$.}.

To summarize the performance of Argus system: in the normal case, which does not involve piracy-reporting or appeal, only $\mathsf{ShareData}$ is involved. In this case, the throughput of Argus system is equal to the throughput of $\mathsf{ShareData}$ ($82.6$ off-chain transactions per second per machine). In the uncommon case of piracy reporting, the throughput of the reporting transactions is $5.0$ tps. In the rare case in which the appeal procedure is performed (i.e., the owner is malicious), the throughput of the appeal transactions is $4.3$ tps. 

% \begin{table}[t]
% \centering
% \caption{Comparison of Performance and Economic Cost between Previous work and Argus}
% \setlength{\tabcolsep}{5pt}
%  \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% Protocols       & \multicolumn{2}{c|}{ReportPiracy} & \multicolumn{2}{c|}{ShareData.Appeal} \\ \hline
% Primitives     & ZKP           & Multi-period      & O(N)-Appeal       & O(1)-Appeal       \\ \hline
% Client Latency & 4.5 s         & 0.354 s           &     45 s (esti.)        & 243.5 ms          \\ \cline{2-5} 
% Economic Cost       & \$ 0.78       & \$ 0.18           & \$ 97 (esti.)         & \$ 0.2            \\ \hline
% \end{tabular}
% \label{tab:perfcompare}
% \end{table}

%\begin{table}[]
%\centering
%\caption{Comparison of informer client latency}
%\begin{tabular}{lll}
%\hline
%Schemes     & ZKP & Argus \\\hline
%Latency (s) & 4.5 & 0.354
%\\\hline
%\end{tabular}
%\label{tab:latency}
%\end{table}

%We also evaluate the off-chain storage cost for Argus. For each transaction between the owner and licensee, the owner and the licensee needs to store some relevant information in $\mathsf{Initiate}$ and $\mathsf{ShareData}$, which costs about 10.6 KB in total. 
% We also evaluate the offchain storage cost for Argus. For each trans, the owner and the buyer needs to store some relevant information about state channel, which costs about 10.6 KB in total.

% Financial cost per report is also evaluated, as shown in Table \ref{tab:price}. The cost is mainly from the gas consumption in Ethereum (similar to transaction fee in Bitcoin). We can find that compared to ZKP scheme, 85.3\% reduction is achieved in Argus mainly because of the use of Multi-period commitment scheme.
%\begin{table}[]
%\centering
%\caption{Financial cost per report}
%\begin{tabular}{lll}
%\hline
%Schemes & ZKP  & Argus \\ \hline
%Payout  & \$0.78 & \$0.22 \\ \hline
%\end{tabular}
%\label{tab:price}
%\end{table}

% The performance and the cost are still feasible with larger N (e.g. N=1000 [*isn't it 10000? -Shuo*]), which is shown in Figure \ref{fig:ot1000}. We can see that only a slight increase in onchain/offchain latency, gas cost when the N increases from 10 to 1000. This implies that we can furthre increase the N to achieve a higher security ( i.e. less probability of frame-up).

% \begin{figure}[thbp]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figs/onchain_latency.pdf}
%     \caption{The performance overhead of Argus when $N=10, 100, 1000, 10000$ }
%     \label{fig:ot1000}
% \end{figure}

% \begin{figure}[thbp]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figs/sharedata_latency.pdf}
%     \caption{The performance overhead of Argus when $N=10, 100, 1000, 10000$ }
%     \label{fig:ot1000}
% \end{figure}

% \begin{figure}[thbp]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figs/storage.pdf}
%     \caption{The performance overhead of Argus when $N=10, 100, 1000, 10000$ }
%     \label{fig:ot1000}
% \end{figure}

% \begin{figure}[thbp]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figs/total_latency.pdf}
%     \caption{The performance overhead of Argus when $N=10, 100, 1000, 10000$ }
%     \label{fig:ot1000}
% \end{figure}

% \begin{figure}[thbp]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figs/gas.pdf}
%     \caption{The performance overhead of Argus when $N=10, 100, 1000, 10000$ }
%     \label{fig:ot1000}
% \end{figure}



==> Argus SRDS Full/instance.tex <==
\section{Implementing the Argus System}\label{sec:construct}

The previous three sections explain the main objectives and the core ideas of Argus. It is important to recognize that the objectives are not separate problems to solve individually. The Argus contract needs to achieve the objectives altogether in a coherent design. Due to the page limit, we only provide a sketch of our construction and implementation here. The holistic view and the implementation details of the Argus system are provided in Appendix \ref{sec:bigpic} and Appendix \ref{sec:imple}, respectively.

With corresponding watermark algorithms, current Argus system supports three data types: image \cite{image}, audio \cite{audio} and software \cite{software}. A Merkle tree structure is leveraged to reduce the on-chain storage: for any list of data, only the Merkle root of the list is uploaded to the blockchain. We also leverage Private Information Retrieval (PIR) \cite{xpir} to reduce the bandwidth overhead of downloading data for the licensees. 

% \subsection{Cryptographic building blocks} 
% In Argus system, we leverage a series of cryptographic primitives, such as Pseudorandom Number Generator (PNG), Oblivious Transfer (OT), Merkle tree, watermarking functions ($E_w$ and $D_w$ for watermark embedding and detection, respectively) and etc. Due to page limit, we move the list of crypto primitives and their formal definitions to Appendix \ref{sec:buildblock}. 

% The security parameter $\lambda$ of these primitives is configurable, which means an adversary could break the primitive with a computation power of O($2^{\lambda}$). With typical $\lambda$ as $128$, the computation power of O($2^{\lambda}$) is considered as impossible. In addition, the number of OT versions $N$ also affects the security of Argus system, which determines the possibility of false accusation (Section \ref{sec:detect}.



% \subsection{A holistic view of the Argus system}\label{sec:brief}

% %\begin{figure}[thbp]
% %    \centering
% %    \includegraphics[width=0.42\textwidth]{figs/mt.pdf}
% %    \vspace{-10pt}
% %    \caption{The three-layered Merkle tree as the core data structure connecting Argus protocols. }
% %    \label{fig:mt}
% %    \vspace{-5pt}
% %\end{figure}

% Due to page limit, we only give a brief descriptions of functions and contracts in the Argus system while details are specified in Appendix \ref{sec:view}.

% The Argus system mainly consists of six protocols: $\mathsf{Initiate}$, $\mathsf{ShareData}$, $ \mathsf{ReportPiracy}$, $ \mathsf{Appeal}$, $\mathsf{ClaimBounty}$ and $\mathsf{ConfirmInfringer}$. These protocols execute between \em{client programs} representing different roles and the \em{contract code} running on the public blockchain. The Argus contract $\mathcal{C}$ includes five functions: $\mathsf{Store()}$, $\mathsf{ VerifyReport()}$, $\mathsf{ VerifyAppeal()}$, $\mathsf{AllocateBounty()}$ and $\mathsf{SetGuilty()}$\footnote{For corresponding contract functions, due to page limits, we omit detailed description here.}.

% $\mathsf{Initiate}$ establishes the basis for the other protocols and contract functions. In $\mathsf{Initiate}$, parameters of OT, watermarked data and targets/bounty for piracy report are prepared. In addition, setup for the information-hiding report (Section \ref{sec:zkw}) is also included. A Merkle tree $rt$ is introduced to reduce the on-chain storage overhead of OTEvidence, which is proportional to $O(N*M)$ ($M$ is the number of licensees). Similarly, $\vec{P}$ in the OT protocol (Figure \ref{fig:ot}) can be also stored on-chain via the Merkle tree proof to avoid the overhead of $O(N)$.

% %\vspace{-10pt}
% $\mathsf{ShareData}$ is the protocol for licensees to obtain data. As described in Section \ref{sec:detect}, the core building block within the protocol is OT adapted for $O(1)$-Appeal. Normally, $\mathsf{ShareData}$ is the protocol invoked most frequently, thus we optimize the on-chain and off-chain bandwidth to make $\mathsf{ShareData}$ more feasible, which is explained in Section \ref{sec:imple}.

% $\mathsf{ReportPiracy}$ is the protocol for the open population to participate in the anti-piracy solution. Thus, we should make this process as cost-efficient and incentive-compatible as possible. The core of this process is the multi-period commitment scheme, which is described in Section \ref{sec:zkw}. In addition, the informer is supposed to fetch some assistant data  (i.e. the Merkle tree path) to generate a transaction to report piracy via $\mathcal{C}.\mathsf{VerifyReport()}$.

% $\mathsf{Appeal}$ can be regarded as the subsequent protocol of $\mathsf{ShareData}$ in case that the innocent Licensee is incriminated by malicious owner in $\mathsf{ReportPiracy}$. From Section \ref{sec:detect}, we can see that only $O(1)$ messages are sent to the contract to invoke $\mathcal{C}.\mathsf{VerifyAppeal()}$ before timeout.
 
%  $\mathsf{ClaimBounty}$ is the protocol for informers to claim the rest of bounty (i.e. $\mathcal{B}_2(n)$ in Section \ref{sec:quantify}) after collection period ends via $\mathsf{AllocateBounty()}$. Note that, the first part of bounty $\mathcal{B}_1(i)$ has allocated upon informers' reveal phase ($\mathcal{C}.\mathsf{VerifyReport()}$).
 

%  $\mathsf{ConfirmInfringer}$ is the protocol for owner to set the status of accused licensee into ``GUILTY'' if the licensee does not successfully appeal during timeout.
% %[*do you plan to finish the description here? I think the description should help readers locate the places where we have novelties, e.g., performance improvements *]

% We further optimize the performance, gas consumption, storage of Argus design, which is introduced in Section \ref{sec:imple}. The evaluation of latency, gas cost can be found in Section \ref{sec:eval}.


%For example, in the $\mathsf{ShareData}$ with a large $N$, since the bandwidth consumption of licensee's downloading data is proportional to $N$, it will considerably increase the latency for the licensee to get the data. Thus, we further apply Private Information Retrieval~(PIR) \cite{xpir} to reduce the overhead. In addition, the overhead of asymmetric encryption/decryption of $N$ versions of data is sidestepped in our scheme. For $\mathsf{Initiate}$, Step 4.d actually impose a significant storage overhead to the owner to store the Merkle tree, which is proportional to $O(M*K*N)$. To reduce the storage overhead, we slightly change $\mathsf{ReportPiracy}$ and allow informers to generate the Merkle tree efficiently. For $\mathsf{VerifyReport}$, which is one of the most expensive contract functions, we use a caching strategy to reduce the gas consumption of this function. During a burst of report submissions, our strategy can significantly reduce the cost of $\mathsf{VerifyReport}$.






==> Argus SRDS Full/intro.tex <==
\section{Introduction}\label{sec:intro}

% Introduction
Intellectual property is one of the most valuable assets for present-day companies, especially in the software, movie, gaming and digital publishing industries. Anti-piracy is a long-lasting and heavily invested effort, because piracy impacts the fundamental business models of these industries. Anti-piracy has the legal aspect and the technological aspect. The former crucially depends on the latter to collect credible and undeniable evidences, so that appropriate legal actions can be taken against the infringers. For example, if evidences prove that the number or the retail value of the pirated copies exceed a certain threshold during any 180-day period, according to the Title 17 of the United States Code, infringers shall be imprisoned for a maximum of 5 years, or fined a maximum \$250,000, or both \cite{title17}.

Since piracy is fundamentally about disseminating copyrighted contents outside legitimate distribution channels, a central question about anti-piracy is how to incentivize people in the open population to report pirated copies. Industrial alliances (BSA \cite{bsa}, FACT\cite{fact}, SIIA\cite{siia}) and companies (e.g., Custos \cite{custos}, Veredictum \cite{veredictum}) have offered big amounts of bounties for piracy reporting. For example, the Business Software Alliance (i.e., BSA \cite{bsa}), whose members include Apple, IBM, Microsoft, Symantec and many others, posted a \$1-million bounty for reporting. However, the approach is not yet effective and is questioned/criticized by the public, mainly due to the lack of transparency \cite{bsanews}. For example, it is unclear whether the \$1-million total bounty is simply a marketing gimmick, as BSA had only rewarded a small fraction of it in a long period of time. Also, BSA's neutrality is really problematic, as its members are copyright holders, who may not represent the best interest of the informers in the public. Moreover, it is unclear how BSA evaluates the credibility of the piracy reports or whether they are strong enough against an infringer's repudiation. Obviously, opaqueness about incentive, fairness, and credibility-criteria seriously limit the effectiveness of these anti-piracy campaigns.

We envision that a methodological progress for anti-piracy campaigns can be made once they are formulated as a decentralized computing problem. It is promising to advance the status quo by distributed-system technologies, especially those about incentive model (NF-Crowd\cite{nf}, Arbitrum \cite{arbitrum}, Hydra \cite{hydra}), consensus mechanism (PBFT-Hyperledger \cite{hyperledgerpbft}, Algorand \cite{algorand}), secure messaging (Decentralized  release \cite{release}, Hyperpubsub \cite{hyperpubsub}, Zerocash \cite{zerocash,zkpcommit}) and Sybil resistance (Arbitrum \cite{arbitrum}, TrueBit \cite{truebit}). Toward the vision, we have built a concrete system named Argus\footnote{Argus (an abbreviation for Argus Panoptes) is a many-eyed giant in Greek mythology, which comprehensively traces misbehaviors.}. The design is based on a clear problem statement and a set of properties as objectives, which are explained next.

\vspace{5pt}
\noindent {\bf Problem statement}. We describe the anti-piracy problem using the following terminology. An {\em owner} is the one who owns the copyrighted content (e.g., a film maker). The content is distributed through a controlled channel to a set of {\em licensees} (e.g., cinemas and film critics). Some licensees may leak their copies of the content, which leads to many pirated copies in the open population. These licensees are called the {\em infringers}. The anti-piracy system's goal is to incentivize people in the open population to report the pirated copies to the system. We refer to these people as the {\em informers}. 

The challenge in the anti-piracy problem is that the interests of these roles are different or even conflicting. Specifically, the owner's goal is to identify infringers and assess the severity of the infringement. The owner wishes that, by giving a financial incentive (e.g., a bounty) to the open population, as many good-faith reports as possible can be received. However, the motivation of informers is not always aligned with the owner. It is only reasonable to assume that informers are financially motivated \cite{arbitrum,nf}, like black-hat security researchers motivated by bug bounties \cite{hydra}. Not surprisingly, an infringer's best interest is to refute the credibility of an evidence by arguing that it could be fabricated by an informer or the owner. 

Because of the conflict of interests, an unbiased solution would require a contract that was agreed upon by all these roles. But who should be the executor of the contract? One possibility is to introduce into the problem an “executor” role, as in the BSA situation described earlier, but the role is really undesirable because its neutrality is hard to be assured in reality (e.g., even big companies like Facebook and Google had controversial practices that put their neutrality in doubt \cite{neutral}). Our work is to explore the feasibility of an open contract of which the execution is fully transparent to the public, without an additional role as the trust basis. 

\vspace{5pt}
\noindent {\bf The Argus system}. In this paper, we present the design, implementation and evaluation of the Argus system. To the best of our knowledge, it is the first public anti-piracy system which (1) does not hinge on any ``trusted" role; (2) treats every participant fairly (in particular, it is resilient to greed and abuse, and resolves conclusively every foreseeable conflict); and (3) is efficient and economically practical to run on a public blockchain (e.g. it achieves an impressive off-chain throughput of 82.6 data-trades per second per machine, and incurs only a negligible on-chain cost  equivalent to sending 14 ETH-transfer transactions per report on the public Ethereum blockchain). 

The four pillars in the Argus design are \textit{full transparency}, \textit{incentive}, \textit{information hiding} and \textit{optimization}. These are the main focuses to be elaborated on in this paper. It is worth noting that they are not four problems to be solved individually, but integral aspects in one coherent design. We highlight some properties of Argus, which represent some of our core innovations:    


\textit{Incentivizing good-faith informers}. A fundamental challenge is about the interest of informers, who are anonymous people in the open population. The owner's interest is to collect good-faith reports so that the severity of the infringement can be accurately estimated. However, each individual informer's interest is to maximize his own reward. What prevents an informer from creating multiple identities to make multiple reports, so that he gets multiple rewards but causes the owner's estimation to be inflated? Note that an attack using multiple forged identities is often referred to as the Sybil attack \cite{arbitrum,truebit}. In Argus, the incentive model ensures that the total reward of the informer and all his Sybils is less than the reward he would get without forging the Sybils. In other words, our model disincentivizes Sybil attacks, so the informers' interest is aligned with the owner's. In addition, our model is superior to previous models because of several other properties for better incentives (Section \ref{sec:quantify}).

\textit{Information hiding for report submission}. Because Argus runs on a public ledger, its execution is fully transparent to everybody \cite{zerocash,zkpcommit}. It is crucial that an informer is unable to resubmit any report previously submitted by somebody else. For this reason, Argus' report submission protocol is based on Multi-period Commitment Scheme, which gives a ``zero-knowledge'' style guarantee, i.e., a submission only proves that the informer has a copy of the content without disclosing other information. Compared to traditional commitment schemes, our scheme leaks no useful information even in the reveal phase while avoiding the heavy cost of zero-knowledge proof (Section \ref{sec:zkw}). 
%This gives a ``zero-knowledge'' style guarantee, i.e., a submission only proves that the informer has a copy of the content without disclosing other information.

%\textit{Timely payout and guaranteed amount}. As mentioned above, Sybil-proofness is crucial for a campaign running in the open population. Previously proposed Sybil-proof incentive models cannot guarantee a reward amount for an informer, who may find the reward arbitrarily low at the end of the campaign. Our incentive model has a guaranteed amount and gives timely payout, which is a better approach to incentivize informers. 

\textit{Strong accusation against infringer}. An owner's accusation against a licensee is always subject to an inherent paradox – since both have the leaked copy, why can't the licensee refute the accusation by arguing that the infringer may be the owner himself? We believe that the only solution to circumvent this paradox is to resort to a probabilistic argument. Argus uses Oblivious Transfer~(OT) to ensure that the false accusation is bounded by a probability $\phi$, which can be arbitrarily small. Hence, the accusation is very hard to refute. Moreover, we improve the efficiency of leveraging OT, which carefully considers the scalability limitation of distributed ledgers \cite{hyperledgerpbft,algorand} (Section \ref{sec:detect}).

%As far as we know, none of existing work can simultaneously achieve above properties. We illustrate that state-of-the-art techniques are trapped in either dilemmas of above properties or limitations of scalability (details in Section \ref{sec:relate}). Our contribution is listed as follows:
% \begin{itemize}
%\item We illustrate a representative scenario of an incentive model for the open population. Other similar scenarios can be quiz bounty \cite{}, non-transfereable sharing \cite{}, etc.
%\item We leverage and adapt state-of-the-art Asymmetric Watermarking to informers and the smart contract for clarify the source of piracy, which generates credible records during data delivering to resolve potential future dispute. 
%\item We introduce Amortized Sybil-proof Bounty with novel properties, such as to keep incentivizing informers with fast payments to report early and honestly.  
%\item We introduce Time-varying Commitment Scheme to counteract replay attack while ensuring fast payments, which is more cost-efficient than ZKP schemes. 
%\item We optimize Argus in performance with specific data structures and protocols. Experiment results demonstrate that Argus can support various data types such as images, audios and software, with sufficient scalability and negligible overhead. The source code and documents of Argus will be publicly available in the near future\footnote{https://github.com/xxx/Argus}.

 %\end{itemize}


 % Compared to previous work, Argus is fully aware of the characters' incentive involved in traitor tracing and leverages blockchain and cryptographic techniques to coordinate characters. As shown in Table \ref{tab:feature}, Argus is advantageous to approach the features of ideal traitor tracing. In addition, Argus is designed to be general for various types of data and scalable in performance/cost. The contributions of this work is as follows:
% we implement Argus which mainly consists of three components: watermarking (embedding, detection), cryptography (OT, Zero-knowledge, PIR, etc.), blockchain (contract, script, etc.). For the first component, without loss of generality, currently we integrate watermarking algorithms of three data types (image, software, AI model) into Argus for demo purpose. For the other two components, we implement corresponding design and evaluate the system on clusters. Experiment results demonstrate that Argus can support various data types with sufficient performance and negligible cost (\autoref{sec:eval}). The source code and documents of Argus will be available in the near future\footnote{https://github.com/xxx/Argus}.

\vspace{5pt}
\noindent {\bf Contributions.} Our contributions are as follows:
\squishlistoneone
\item We formulate anti-piracy as a problem about consolidating different interests of multiple roles, including informers in the open population. We also clearly state the design objectives of anti-piracy solutions, which give a foundation for this work and future research.
\item The Argus contract is fully transparent --- no role is considered as the trust base. This is a significant advancement. In addition, our approach is systematic. Because of the clarity on the design objectives, we are able to deduce the general form of the incentive model and identify all the unavoidable technical challenges. Because these challenges are general, solving them in Argus will have a far-reaching impact in the broad problem space. 
\item To achieve full transparency and a number of novel objectives, Argus needs to implement sophisticated cryptographic operations as contract code, rather than native code. Optimizations are a vital effort in the design of Argus. We show that, if existing cryptographic operations were adopted without optimization, the cost would equal sending thousands of transactions (as opposed to 11 transactions in Argus), which would make the solution economically unreasonable. 
\squishlistoneoneend

\noindent {\bf Roadmap}. The rest of the paper is organized as follows. Section \ref{sec:basicargus} gives an overview of Argus to address how we leverage a transparent contract to achieve the mutual trust and fairness between owner, licensees and informers, along with related primitives. In Section \ref{sec:quantify}, Section \ref{sec:zkw} and Section \ref{sec:detect}, we further figure out that those primitives should be optimized to achieve four pillars with better practicality. Then, we brief our implementation with optimizations in Section \ref{sec:construct}. In Section \ref{sec:eval}, the security analysis and performance evaluation of Argus are provided, followed by related work in Section \ref{sec:relate} and a conclusion. The Appendix provides details of mathematical deduction, protocol implementations and security analysis.  
 


==> Argus SRDS Full/overview.tex <==
\section{Overview of Argus} \label{sec:basicargus}
In this section, we give an overview of the anti-piracy solution and Argus contract. We assume familiarity with contract \cite{solidity} and cryptographic primitives such as oblivious transfer \cite{np}, zero-knowledge proof \cite{zksnark} and commitment scheme \cite{commitment}. 

\subsection{The Argus Contract} 
Figure \ref{fig:overview} illustrates the important elements in the Argus contract and how different roles interact with it. 
An instance of the Argus contract is created by the owner of a copyrighted content. We denote $M$ as the number of licensees and list the data fields used in the Argus system in Table \ref{tab:data}.
%\vspace{-10pt}
\begin{table}[b]
\vspace{-15pt}
\footnotesize
\centering
\caption{Data fields used in the Argus system}
\setlength{\tabcolsep}{1pt}
 \renewcommand{\arraystretch}{1.1}
\begin{tabular}{|l|l|}
\hline
Data fields           & Description                                                                                                                                                              \\ \hline
\textrm{LicenseeStatus[$M$]} & \begin{tabular}[c]{@{}l@{}}To store the status of every licensee. Each \\ status belongs to set \{NORMAL, ACCUSED, \\ GUILTY, EXONERATED\}\end{tabular} \\ \hline
\textrm{OTEList[$M$]}        & \begin{tabular}[c]{@{}l@{}}To store the OTEvidence of every OT between\\ owner and Licensee\end{tabular}                                                            \\ \hline
\textrm{ReportNumber[$M$] }  & \begin{tabular}[c]{@{}l@{}}To indicate the number of leaked copies from\\ every licensee by counting informers' reports\end{tabular}                                      \\ \hline
\end{tabular} \label{tab:data}
% \vspace{-15pt}
\end{table}

\begin{figure}[t]
% \vspace{-15pt}
    \centering
    \includegraphics[width=0.43\textwidth]{figs/overview.pdf}
    \vspace{-5pt}
    \caption{Overview of the Argus system. }
    \label{fig:overview}
    \vspace{-20pt}
\end{figure}


When the owner distributes the content to the licensees, she generates a large number of watermarked copies, e.g., $10000*M$ copies. In other words, each copy is embedded with a unique secret string. In this work, we assume that nobody can remove the watermark from a copy without badly deteriorating the content quality. Despite this assumption, we will describe in Section \ref{sec:model} our insights about improving the robustness of watermark.

A licensee retrieves a copy from the owner through oblivious transfer (OT), which ensures: (1) the owner does not know which of the watermarked copies is retrieved; (2) the licensee knows nothing about other copies except the retrieved one. The OT procedure is performed by private computations on the owner side and the licensee side. One of our important features added to the existing OT protocol is to produce a data record called {\em OTRecord} on the licensee side, which is needed in case the licensee appeals against an accusation. In addition, the OT scheme produces another piece of data called {\em OTEvidence}, which opaquely represents the existence of the current OT procedure. Every OTEvidence is submitted to the contract via function \texttt{CommitEvidence(OTEvidence)}. The set \texttt{OTEList[M]} defined in the contract stores all OTEvidences. 

Suppose a copy of the content is leaked out into the open population. In Figure \ref{fig:overview}, we assume that informer$_X$ gets the copy and wants to report. The informer should first extract the secret string from the watermarked copy. The reporting is to fulfill an information-hiding procedure to show informer's acquaintance of the secret string, which is via function \texttt{Report(ProofOfLeakage)} of the contract and increases an element of \texttt{ReportNumber[M]}.  
Function \texttt{Report()} can be either implemented via commitment scheme or zero knowledge proof.
% [* say something about ProofOfLeakage -shuo*].
Because \texttt{Report()} is an information-hiding procedure, other people in the population cannot learn anything about the watermarked copy reported by informer$_X$, thus cannot report about the same copy unless they actually have it.
Nevertheless, the information-hiding submission does not prevent informer$_X$ from creating multiple Sybil identities to submit multiple reports about one watermarked copy. Function \texttt{Reward()} of the Argus contract implements an incentive model that causes the total reward obtained through the Sybil attack to be less than what the informer would normally receive. We will explain the incentive model in Section \ref{sec:quantify}. Function \texttt{Reward()} is periodically invoked according to the ledger's clock so that informers can get timely rewards.

Once a report is received by the contract, the reported copy will reveal which licensee is accused and update\texttt{ LicenseeStatus[M]}. The status of the licensee is changed from NORMAL to ACCUSED. The licensee has a time period for appeal. If he does not call function \texttt{Appeal(OTRecord)} within the period, function \texttt{SetGuilty()}, also invoked by the owner according to the ledger's clock, changes the licensee's status to GUILTY. If he calls \texttt{appeal(OTRecord)} within the period, the OTRecord will reveal which watermarked copy the licensee received via OT. If it is the same copy revealed by the report, the licensee's status is changed to GUILTY. Otherwise, it is changed to EXONERATED. Once exonerated, this licensee is exonerated for this copyrighted content, because the identity of his copy has been disclosed. 

There are different ways to implement the Argus contract, but every solution should include three elements: (1) an {\bf\em incentive model}, (2) an {\bf\em information-hiding submission scheme}, and (3) an {\bf\em OT scheme}. Before presenting these elements in following sections, we introduce the trust assumptions of Argus below.
% However, there are also some challenges to address since participants may betray from above steps to maximize their profits:
% \begin{itemize}
% \item {\bf Copy attack.} As shown in Figure \ref{fig:model} (c), due to the transparency of blockchain, ever since a informer reports privacy/leakage to the contract, other informer may copy the report. The nodes within the blockchain network may launch front-running attack during the propagation of the first informer's report. In Section \ref{sec:zkp}, we will show how to leverage zero-knowledge proof to address the attack. 
% \item {\bf Sybil attack.} As shown in Figure \ref{fig:model} (d), informers may repeatedly submit the answer themselves or via other informers. In addition, informers may redistribute the pirated/leaked data since they are free of charge\cite{}. A promising solution is Syble-proof bounty \cite{arbitrum}, which incentivise the informers not to re-submit or redistribute the data. In Section \ref{sec:spb}, we will show the limitation of previous sybil-proof bounty and propose a novel mechanism. 
% \item {\bf Frame-up attack.} As shown in Figure \ref{fig:model} (b), since the owner knows the watermarked data delivered to any licensees, the owner may incriminate the innocent licensees. Previous work have proposed Asymmetric watermarking (so-called Buyer-seller watermarking) to mitigate the frame-up attack \cite{ot1,ot2}. In Section \ref{sec:detect}, we will demonstrate that the overhead and the incentive of Asymmetric Watermarking can be further optimized. 
% \end{itemize}

% In Section \ref{sec:analysis}, we will analyze the security of Argus. With countermeasures to above attacks and previous attack model, we will prove that Argus surpasses existing solutions from incentive-compatability and attack-resistance defined in Section \ref{sec:relate}.

\subsection{Trust Assumptions} \label{sec:model}
We make three trust assumptions for the design and evaluation of Argus.
\squishlistoneone
\item{\bf Robust watermarking.} We assume watermarking cannot be compromised without considerable degradation of the content's value. Existing work has shown success of watermark robustness in certain domains. For example, the image watermark can protect against attacks such as splitting, sampling, filtering, image compression \cite{image}. Although novel attacks such as oracle attack \cite{sensitivity} and collusion attack \cite{bscode} emerge, watermark techniques keep evolving with new countermeasures \cite{sensitivity2,tardos}. We see this as a separate research concern.
\item{\bf Financially motivated informers.} We assume that a financial reward is the only motivation for every informer \cite{arbitrum, truebit} . This implies that, if an action results in a loss of reward, no informer will take the action. % In addition, we do not consider informers' profits elsewhere outside Argus.
%Participants (owner, licensee, informer) may take any malicious actions to maximize their own profits. Previous work assume participants are honest by default. For example, they assume that the owner will not cheat informers to deny their rewards. However, the dispute between owner and informer is prone to occur even if the owner is honest as long as the owner is centralized and ``black-box''. In addition, the owner/informer may incriminate the innocent licensee or repeat the whistleblowing to overpunish the licensee, which is not discussed by previous work. Consequently, we hope to ensure the functionality of Argus under a more realistic assumption.  
\item{\bf Trusted blockchain.} We assume the trustworthiness of the blockchain. There are technologies to enhance security at the ledger layer \cite{pow,pos} and the smart contract layer \cite{teether,oyente,zeus,paymentprotect}. We also see this as a topic complementary to Argus.
\squishlistoneoneend

%Except for above three assumptions, we assume that the cryptographic techniques involved in this work, such as Oblivious Transfer \cite{np}, Private Information Retrieval \cite{xpir} and Zero-knowledge Proof \cite{zksnark} are secure under certain assumptions. Their security is comprehensively studied which is out of the scope of this paper.

==> Argus SRDS Full/pre.tex <==
\section{Preliminaries}\label{sec:pre}
\subsection{Primitives}
{\em Secure watermarking}\cite{image,audio,software,dnnwatermark}. For simplicity, we formulate the digital watermarking system as a tuple $(x, y, id, E_W, D_W)$, where ${x, y, id, E_W, D_W}$ denotes original/watermarked data, embedded ID, watermark embedding/detection algorithm, respectively. They have the following relationship: $ y = E_W (x, id), id = D_W (y)$. Two important features of secure watermarking are {\em robustness} (even if $y$ is considerably modified as $y'$,  $D_W (y')$ still equals $id$) and {\em security} ($D_W$ can conceal relevant information to prevent attackers from directly removing watermark).

Unfortunately, even if a buyer is traced and incriminated via watermark detection results, the user may deny the guilt or significance of piracy since the seller and third-parties can also redistribute the watermarked data leading to a frame-up or an overestimate. Consequently, the disputes may stagger later copyright enforcement unless further evidence is provided.   

To address the dispute, {\em asymmetric watermarking} (so-called buyer-seller watermarking \cite{ot4}) is proposed and investigated \cite{ot1,ot2,ot3}. In early work, secure multiparty computation \cite{tt2} and homomorphic encryption \cite{ot4} are proposed to generate watermarked data without seller's knowing the data, which are considered too expensive in practice \cite{ot1}. Consequently, state-of-the-art work leverage Oblivious Transfer (OT) \cite{np,otorigin} which is much more efficient in performance \cite{ot1,ot2,ot3}: the seller generates $N$ copies of data watermarked with different unique IDs and plays OT protocol with the buyer. Then, the user can obtain only one copy without owner's knowing which one. Thus, when there is a dispute, the seller and the buyer can refer to a {\em judge} providing related evidence. In Section \ref{sec:detect}, we will further improve asymmetric watermarking in cost/scalability.
\subsection{Blockchain}
Blockchain is a distributed ledger system running on nodes among a P2P network. With the combination of consensus protocol and cryptography, nodes can execute programs with a same logic to reach consensus about the ledger states without trusting each other. In the P2P network, nodes send or propagate signed transactions to or from other nodes. Moreover, nodes are supposed to record and validate every transaction in order to ensure the correctness of its local ledger. When divergence occurs, consensus protocol functions, such as proof-of-work (POW) \cite{bitcoin}, proof-of-stake (POS) \cite{mauve}, PBFT \cite{pbft} and Raft\cite{raft}. 
%Above protocols all depend on ``votes'' from the distributed nodes while ``votes'' vary in forms for different consensus protocols. 

%The form of the vote highly relates to the type of the blockchain. In {\em public blockchain} such as Bitcoin \cite{bitcoin} and Ethereum \cite{ethereum}, every node is free to vote. Thus, in order to mitigate the risk of Sybil attack \cite{pbft}, computation power (i.e. POW \cite{bitcoin}) or stake (i.e. POS \cite{mauve}) is required to increase the cost of vote. By contrast, in {\em permitted blockchain}, such as Hyperledger \cite{hyperledger} and Corda \cite{corda}, only permitted node can vote. With this constraint, PBFT is enough to guarantee the consistency of blockchain data. With additional conditions, Raft can be used \cite{coco}. As a consequence, permitted blockchain is considered to be more efficient in performance with less decentralization compared with public blockchain. 

%which is first proposed by Satoshi Nakamoto in 2009 \cite{bitcoin}. 
%With the combination of consensus protocol and cryptography, nodes can execute programs with a same logic to reach consensus about the ledger states without trusting each other. In the P2P network, nodes can send or propagate signed transactions to or from other nodes. Moreover, nodes are supposed to record and validate every transaction in order to ensure the correctness of its local ledger. When divergence occurs, consensus protocol functions, such as proof-of-work (POW) \cite{bitcoin}, proof-of-stake (POS) \cite{mauve}, PBFT \cite{pbft}, Raft\cite{raft}. Above protocols all depend on ``votes'' from the distributed nodes while ``votes'' vary in forms in different consensus protocols. 
%
%The form of the vote depends on the type of the blockchain. In public blockchain such as Bitcoin and Ethereum, every node is free to vote. Thus, in order to mitigate the risk of Sybil attack \cite{pbft}, computation power (i.e. POW \cite{bitcoin}) or stake (i.e. POS \cite{mauve}) is required to increase the cost of vote. By contrast, in permitted blockchain, such as Hyperledger \cite{hyperledger} and Corda \cite{corda}, only permitted node can vote. With this constraint, PBFT is enough to guarantee the consistency of blockchain data. With additional conditions, Raft can be used \cite{coco}.

The above mechanisms lead to one most important feature of blockchain system called {\em decentralization}, which means the ledger is not secured by a centralized authority but distributed nodes. To extend the forms of decentralized trust and facilitate complicated applications over blockchain, script system \cite{bitcoin} or smart contracts \cite{ethereum} are introduced to support functionalities such as freezing/unfreezing funds, time-stamping, etc. These functionalities further enable a variety of applications which requires high confidence of trust, such as blockchain-based bounty system. 

Bounty systems have been demonstrated efficient in various scenarios such as program bug \cite{}, software piracy \cite{}, etc. However, the uncertainty of risking nonpayments can considerably undermine third-parties' incentives of cooperation. As a result, blockchain-based bounty mechanism are widely proposed with enforcement of rewarding, which is similar to that of blockchain-based exchange protocol \cite{fairswap}.

For example, to collect the watermarked data for detection, it is believed that the seller should cooperate with bounty hunter to circumvent technical obstacles \cite{presentation,custos}. Custos \cite{custos}, which is most related to our work, has proposed to design watermarked information as the private keys of different cryptocurrency accounts with balance. Consequently, any well-informed piracy users would extract the information to obtain certain accounts' balance, which leads to an on-chain transaction. The transaction can indicate corresponding illegal buyers and serve as evidence for further forensics and judgments. In summary, the blockchain-based incentive mechanism has enabled a credible threat to deter users from redistributing pirated copies. Similarly, Veredictum \cite{veredictum} has proposed to incentivise third-parties as crawlers for piracy copies through a bounty contract \footnote{According to Veredictum's latest whitepaper, current implementation does not leverage watermark \cite{Veredictumpaper}.}. 

Blockchain-based bounty is also leveraged in other scenarios. For example, Hydra \cite{hydra} has proposed to attract experienced hackers to submit bugs of valuable contract via blockchain-based bounty. They also propose commit-and-reveal with submarine commitment to mitigate front-running attack in blockchain. Arbitrum \cite{arbitrum} has proposed an efficient trusted off-chain computation mechanism based on the supervision of third-parties incentivized by blockchain-based bounty.
\subsection{Sybil attack}
Incentive mechanism
\subsection{Related Cryptographic Primitives}
In this section, we briefly introduce three cryptographic primitives involved in Argus: Oblivious Transfer and Private Information Retrieval.
\subsubsection{Oblivious Transfer} 
A $K$-out-of-$N$ Oblivious Transfer (OT) between an owner and an user is a cryptography protocol which guarantees following two properties:
\begin{itemize}
\item The user can arbitrarily choose $K$ data to obtain from $N$ candidate data. The user cannot know the unchosen data.
\item The owner cannot know which $K$ data are chosen by the user.
\end{itemize}

\begin{figure*}[thbp]
\fbox{
\pseudocode{%
\textbf{ Owner} \< \< \textbf{ User}  \\[0.1\baselineskip][\hline]
 \<\< \\[-0.5\baselineskip]
\{C_i\} \sample \ZZ_q \< \< \\
r \sample \ZZ_q \< \< \\
 R \gets r\cdot G \ \<\< \\
\{C'_i\} \gets \{r \cdot C_i\}\\
 \< \sendmessageright*{\{C_i\},R} \< 
\pclb
 \pcintertext[dotted]{Initializing Phase Ends} 
  \<\< k \sample \ZZ_q \\
 \<\< j \sample\set{1,\ldots,N} \\
 \<\< PK_0 \gets C_j-k \cdot G \pclb
 \pcintertext[dotted]{Choosing Phase Ends} 
 \< \sendmessageleft*{PK_0} \< \\
 PK'_0 \gets r\cdot PK_0 \ \<\< \\
 r\cdot PK_i \gets C'_i-PK'_0 \<\< \\
 \{E_i\} \gets \{H(r\cdot PK_i, R, i) \oplus M_i\} \<\<\\
 \< \sendmessageright*{\{E_i\}} \< \pclb
 \pcintertext[dotted]{Transferring Phase Ends} 
 \<\< M_j = E_j \oplus H(k \cdot R, R, j) \\
 }
 }
 \centering
\caption{Basic OT \cite{np}} \label{fig:ot}
\end{figure*}



OT have many implementations and optimizations \cite{ote,np,otorigin,simple}. Without loss of generality, we adopt Naor-Pinkas $1$-out-of-$N$ protocol in this work \cite{np}, which is illustrated in Figure \ref{fig:ot}:
%$N$ messages $M_1,M_2,\dots,M_N$
\begin{enumerate}
\item {\bf Initialize .} The owner generates $N$ random points $ \{C_i \in  Z_q\} (1\le i \le N)$ and a random number $r$. Then, $ \{C_{i} \}$ and $R=r\cdot G$ are published. The owner also precomputes $\{r \cdot C_{i} \}$.
\item {\bf Choose.} The user chooses a random number $k$ and an arbitrary index $j$ within $\{1,2,\dots,N\}$. Then, the user calculates $PK_0=C_j-k\cdot G$ which is then sent to the owner. 
%and records $PK_0$ in the contract.
\item {\bf Transfer.} The owner calculates $r \cdot PK_0$ and calculate $r\cdot PK_i=r\cdot C_{i}-r \cdot PK_0$ with precomputed $\{r \cdot C_{i} \}$. Then, $\{H(r\cdot PK_i, R, i) \oplus M_i\}$ are sent to the user. Since the user can calculate $k \cdot R$ which equals $r\cdot PK_j$, the user can obtain chosen data $M_j = (H(r\cdot PK_j, R, j) \oplus M_j) \oplus H(k \cdot R, R, j) $.
\end{enumerate}




% \subsubsection{Zero-knowledge Proof}
% Zero-knowledge proof (ZKP) is a cryptography protocol used in various systems \cite{zerocash,arbitrum,hawk}. ZKP can be represented by a tuple $(P,V,a,w)$ where $P/V$ denotes proving programs/verifying programs and $a/w$ denotes public input/secret witness of the prover. ZKP should have following three properties:   
% \begin{itemize}
% \item {\bf Completeness.} If the prover knows $w$, then the prover can generate a proof which can be validated by the verifier: $Pr[V(a,P(a,w))=0] = negl(\lambda) \label{eq:zkp}$
% \item {\bf Soundness.} If the prover does not know $w$, then the prover cannot generate a valid proof with a fake $w'$: $Pr[V(a,P(a,w'))=1] = negl(\lambda) \label{eq:zkp}$
% \item {\bf Zero-knowledge.} The verifier cannot learn anything from the proof of the prover.
% \end{itemize}

% $P/V$ can be either interactive \cite{interactive} or non-interactive \cite{zksnark}. And state-of-the-art ZKP introduce an another powerful property called {\em succinctness}. ZKP with succinctness, such as zk-SNARK \cite{zksnark}, can generate a fixed-length proof in bytes for arbitrary programs, which enables enormous scenarios and applications. In Section \ref{sec:zkw}, we will leverage ZKP to protect whistleblowers' report from being copied by others.
% %zk-SNARK to generate the binary of prover's program with verifier's logic in the contract.

\subsubsection{Private Information Retrieval}
Private Information Retrieval (PIR) is similar to Oblivious transfer except that in PIR the user is allowed to obtain all candidate data. The optimization goal of PIR is that the user can obtain intended data with negligible computation/communication overhead of both sides of owner/user. Various implementations of PIR have been shown \cite{xpir} and state-of-the-art PIR scheme are based on homomorphic encryption \cite{pir1,pir}. As one of state-of-the-art work, XPIR leverages Ring-LWE encryptions \cite{ring} and have demonstrated sufficient performance \cite{xpir}. To mitigate the bandwidth problem in asymmetric watermarking, we will use XPIR as a stand-along module in Section \ref{sec:imple} and thus do not introduce XPIR's details. \footnote{For details of XPIR, please refer to \cite{xpir} and code repo \cite{xpirrepo}}. 

==> Argus SRDS Full/quantify.tex <==
\section{Incentive Model}\label{sec:quantify}
As mentioned in the introduction, an incentive-compatible mechanism is required in Argus. It is a challenge because of the open population --- the owner does not know the real-life identities of informers. The interests of the owner and the informers are different: the owner wants to receive good-faith reports, and the informers (both honest ones and greedy ones) want to get financial rewards. The goal of the incentive model is to consolidate these different interests.
The design of our incentive model is inspired by some models in the literature \cite{arbitrum,truebit}. However, because we have the target problem clearly formulated (as in the introduction), we are able to deduce a general form of the incentive model. Our approach is superior for three reasons: (1) it is unclear how the incentive models in the literature were obtained. They seem more of a ``creative art'' than a result of a disciplined design; (2) our general form encompasses all models that satisfy the incentive objectives of all roles. The existing models in the literature are simplified special cases of our general form; (3) our model ensures extra desirable properties, such as {\em timely payout} and {\em guaranteed amount}, which we see as very important aspects of informers' incentive.
\subsection {The Objectives of Incentive Models} \label{sec:modelobj}
Before introducing our general-form model, it is worth making explicit the objectives of a desirable incentive model.
\squishlistoneone
\item First, the model must {\em disincentivize Sybil attacks}. It is easy to understand that, due to the open population, any informer can create multiple identities (i.e., Sybils), so it is not possible for the owner to detect Sybil attacks. Hence, an objective of the incentive model is to disincentivize them, so that the total reward of all Sybils of a duplicate report is lower than the reward of a single unique report. With this property, an informer (who is assumed to be financially motivated) will not inflate the owner's counts in \texttt{ReportNumber[]}.
\item Second, it is the owner's interest to {\em incentivize timely reports}, so an informer reporting earlier should be rewarded more than another one reporting later. Essentially, under the incentive model, informers are competitors racing against time. Nothing can be gained by delaying a report.
\item Third, it is the informers' interest to {\em get timely payouts} and {\em guaranteed amounts}. In all existing models, informers need to wait until the end of the campaign to know the amounts and get the rewards. We believe that a good incentive should reward an informer shortly after the report is confirmed valid. The time to reward should be independent of the campaign's duration. 
%In addition, a guaranteed amount protects an informer's incentive from a malicious owner (Section \ref{sec:analysis}).
 \squishlistoneoneend

\subsection{Deducing the Reward Function from the Objectives}
We formulate the incentive model as a reward function $B(I_i,n)$, which denotes the bounty value for the $i$-th successful informer $I_i$ (informers are chronologically ordered) when the total number of informers is $n$. Previous proposals have given a special form of $B(I_i,n)$ as $c*2^{-n+1}$ ($c$ is a constant denoting the total bounty value) under certain constraints \cite{arbitrum}, but they have not formalized the properties of $B(I_i,n)$ {\em in a general form}. %, leading to a limited expression of $B(I_i,n)$. 
For example, the work \cite{arbitrum} only gives the special form with the assumption that $B(I_i,n)=B(I_j,n) (i \neq j)$, i.e., every informer's reward is equal. 

In this paper, we go through the process of deducing the reward function from the objectives. The mathematical definitions of the properties corresponding to aforementioned objectives are as follows:
\squishlistoneone
\item {\bf Sybil-proofness.} Arbitrary subset of informers get a reduced total reward if the total number of submissions increases: $ \sum_{i \in S_m} B(I_i,m) \ge \sum_{i \in S_k} B(I_i,k) $,  where $m \le k$ are two positive integers and $S_m \subseteq S_k$ are two arbitrary subsets of $\set{1,\ldots,m}$ and $\set{1,\ldots,k}$, respectively. 
\item {\bf Order-awareness.} The earlier the informer reports, the more bounty he/she obtains: $B(I_i,n) \ge B(I_{i+1},n)$.
\item {\bf Timely payout.} Each informer is rewarded in an amortized style: $B(I_i, n) = B_1(i)+B_2(n)$, where $B_1(i)$ is only related to $i$, so the reward can be paid immediately.
\item {\bf Guaranteed amount.} An informer, upon a confirmed reporting, is guaranteed a minimal reward amount $c_{i}>0$, i.e., his/her total reward will not be under $c_{i}$ as the number of informers increases: $\lim_{n \rightarrow \infty} B(I_i, n) \ge c_{i}$.
\squishlistoneoneend

Note that except for the first property, the others are not achieved by reward function $B(I_i,n) = c*2^{-n+1}$ from previous work. We ascribe the limitations of previous incentive models to the lack of a general-form deduction, which is addressed in our work. Due to the page limit, we move the mathematical deduction for the general form and the process of enriching properties to Appendix \ref{sec:math}. We only highlight the final expression of $B(I_i,n)$, which can be formalized as Theorem \ref{th:expr}:

\begin{theorem}[\bf The expression of $B(I_i,n)$] \label {th:expr}
To satisfy Sybil-proofness, Order-awareness, Timely Payout and Guaranteed Amount, $B(I_i,n)$ should satisfy following equation:

\begin{equation} \label{eq:gf}
 B(I_i,n) = -\xi_i+\sum_{j=i+1}^n \xi_j+c*2^{-n+1}
 \vspace{-15pt}
\end{equation}
{\small
 \begin{eqnarray} \label{eq:p1}
 \nonumber \textrm{\normalsize where }
  \xi_{i+1}=\sum_{j=1}^{i} 2^{j-i}*\Delta_j\  ,\quad
  \sum_{j=1}^{\infty} 2^{j}*\Delta_j \le c ,\quad
  \set{\Delta_i} \in  \mathbb{R}^{*}_{\ge 0}
 \end{eqnarray}
 }
 \end{theorem}



\subsection{Plugging in real-world numbers}

In the introduction, we describe the \$1-million USD campaign opaquely run by the BSA \cite{bsanews}. After a long period of time, only a small percentage of the total amount was paid out to informers. This is obviously a low incentive to the public. We now analyze the outcome if Argus is used for the \$1-million USD campaign. We instantiate the parameters $\Delta_i=2^{-i}*c/l \textrm{ } (\textrm{for } i=1,\ldots,l) \textrm{ or } 0 \textrm{ }(\textrm{for } i>l)$ in Theorem \ref{th:expr} where $l$ can be an arbitrary positive integer. For simplicity, we set $l=20$ in this work, which is a typical boundary to classify copyright infringement \cite{title17}. With this setting, we compare Argus with previous work \cite{arbitrum,truebit}, which are also Sybil-proof models.

Figure \ref{fig:instance} shows the reward amount (in the log scale) that each of the n informers will get in our incentive model (the upper diagram) and the previous model (the lower diagram). Every line in the lower diagram is horizontal, because the previous model does not have order-awareness. As a result, all informers get the same reward, and the reward is exponentially decreased with n, in order to ensure Sybil-proofness. There is no guaranteed amount when a report is confirmed. When the campaign ends, even an early informer may find the reward almost zero if there are many later informers. It is a problematic model to incentivize people.

The upper diagram shows our model. The line of $n=\infty$ corresponds to the guaranteed amounts for the informers. Our lines are also affected by n, but not as drastically as in the previous work. As n increases, the lines become closer to the $n=\infty$ line (note that the n=100 line is visually overlapped with it), suggesting that every existing informer loses some reward when a new informer joins. The design of our reward function ensures that the loss of reward is big enough so that no informer wants to fake a Sybil identity to get another reward.  

Compared to the (problematic) incentive shown in the lower diagram of Figure \ref{fig:instance}, the reward function of Argus is superior in all objectives we set in the beginning of this section. 
%We can see from the figure that our incentive model is superior to those in the existing proposals:
%\begin{itemize}
%\item {In our model, the early informers get very significant rewards, with the first reward \$65625, 40625, 28125 and the 10th reward \$585.75. These amounts are not affected by the number of future report submissions. For the incentive model of the previous work, if the total number of valid reports n is 5, everyone get \$62500; if n is 10, everyone gets \$1953. There is no guaranteed amount when a report is confirmed. }
%\item {Regardless of n, our incentive model gives out over 10\% to the informers, whereas the previous work only gives out 31.3\%, 19.5\% and 3.8*$10^{-5}$ of the \$1M when n is 5, 10 and 20, respectively. These are very small incentives, resulting from the Sybil-proofness design of the previous work. Since the public complained about the BSA campaign for the small actual payout \cite{bsanews}, the incentive model in the previous work will face the similar issue when deployed in the public.}
%\end{itemize}



%With Equation \eqref{eq:instancetotal} and assumption that $c=\pounds 1000 $ \cite{fact}, we can compare our incentive model from previous work \cite{arbitrum,truebit} in which $B(I_i,n)=c*2^{-n+1}$. In Figure \ref{fig:instance}, we illustrate the reward value of first five informers in our incentive model and previous work, respectively. Since every informer gets the same value of reward, we simply illustrate one bar (``Previous Work'') to present previous incentive model. We can find that in previous incentive model, the reward value of informers turns negligible if $n$ is sufficiently large. By contrast,  in our incentive model, since the total reward of every informer is mainly determined by the timely payout part (i.e. $B_1(i)$), the total reward is nearly not affected by the increasing $n$.


\begin{figure}[thbp]
    \vspace{-10pt}
    \centering
    \includegraphics[width=0.43\textwidth]{figs/instance.pdf}
    \caption{The reward of first twenty informers in (a) our incentive model and (b) previous incentive model \cite{truebit, arbitrum}, respectively (when total number of informers $n=5,10,20,100$). }
    \label{fig:instance}
    \vspace{-0pt}
\end{figure}

%\begin{figure}[thbp]
%    \centering
%    \includegraphics[width=0.45\textwidth]{figs/total.pdf}
%    \caption{The total reward of all informers with different $n$. }
%    \label{fig:ins}
%\end{figure}

\noindent\textbf{Further improving the incentive.} It is worth to acknowledge that Sybil-proofness imposes an intrinsic property of the reward function --- it must decrease exponentially to foil a Sybil attack (see Corollary \ref{co:1} for details). The previous model, our model and future models are all constrained by this bound. For example, in our model, if n=20, the $1$st, $5$th, $10$th and $18$th informers get the reward amounts of \$ $100000$, \$$6250$, \$$196$ and \$$1.07$, respectively. For informers who report too late, if they inspect the blockchain to figure out their indices, they may not see enough incentives. Hence, to further improve the incentive model, a new objective is to conceal the actual number of submissions in blockchain transactions with techniques such as the unlinkable anonymous payment\cite{zerocash} and the submarine commitments \cite{hydra}. When this is achieved, every informer will have the equal hope that he/she may win the first (largest) reward, since the blockchain log reveals no information in this regard. We leave the design and implementation as future work.

%With the feature of amortized allocation, we can set a much more flexible deadline mechanism in the contract to lengthen the protection period of the data compared to the fixed time-based mechanism. For example, we can set the terminal condition as $N_{report}>N_{th}$ where $N_{report}$ denotes the number of successful reports and $N_{th}$ denotes a certain threshold. In Section \ref{sec:analysis}, we will see by this deadline mechanism, our sybil-proof bounty is immune to commitment contract \cite{threat}.
%
%In Section \ref{sec:eval}, we will quantitatively compare our incentive model with previous work to illustrate the better incentive. 



% \subsection{Time-aware Incentive Model}
% As described in previous section, the equation \eqref{eq:aspb} achieves the property of amortized allocation. This, however, may bring a new challenge:  users may launch sybil attack in order to early withdraw the $\sum_{j\ge i} B_1(j)$ since the interest of these bounties can be used 

==> Argus SRDS Full/relate.tex <==
\section{Related Work}\label{sec:relate}
 
% \noindent{\bf Bounty Incentives.}
% Bounty systems have been carried out in various real-world scenarios such as security bugs \cite{hydra}, software piracy \cite{bsa,siia,fact}, verifiable contract execution \cite{truebit,arbitrum} and crowdsensing \cite{crowdsense}. Recently, blockchain-based bounty mechanism emerges. 
% For example, Custos \cite{custos}, which is the most related work, proposes to design watermarked information as the private keys of different cryptocurrency accounts with balance. Consequently, any informers would extract the information to obtain certain accounts' balance, which leads to an on-chain transaction. The transaction indicates the corresponding infringer and facilitates future forensics and judgments. However, Custos cannot quantify the number of copies of a pirated content. It is unable to make a strong accusation that resists the infringer's repudiation. 
% %In summary, the blockchain-based incentive mechanism has enabled a credible threat to deter users from redistributing pirated copies. Similarly, Veredictum \cite{veredictum} has proposed to incentivize third-parties as crawlers for piracy copies through a bounty contract.
% % \footnote{According to Veredictum's latest whitepaper, current implementation does not leverage watermark \cite{Veredictumpaper}.}. [*need Xian's explanation to revise this paragraph *]
% Blockchain-based bounty is also leveraged in other scenarios. For example, Hydra \cite{hydra} proposes to attract experienced hackers to submit bugs of valuable contract via blockchain-based bounty. Arbitrum \cite{arbitrum} proposes an efficient trusted off-chain computation mechanism based on the supervision of third-parties incentivized by sybil-proof bounty.

% \noindent{\bf Digital Watermarking.}
% Digital watermarking is widely proposed as a reinforcement to the copy protection system. Watermark is a piece of data embedded in valuable data to address potential disputes of copyright, which can be leveraged by future forensic/judgments. Watermark is usually designed to be imperceptible to applications and robust to a wide range of distortion/attack \cite{image,audio,dnnwatermark}. Previous work proposed watermarking schemes for various forms of traditional data such as multimedia (images \cite{image}, audios \cite{audio}, videos \cite{video}), database \cite{sql}, documents \cite{custos} and software \cite{software}, along with emerging data types such as AI models \cite{dnnwatermark}. Furthermore, seller can associate the watermark with licensees' ID before embedding, which enables to trace infringers \cite{fingerprint,ot1}.  


% A category of watermarking technologies, namely {\em asymmetric watermarking} (AWM, so-called buyer-seller watermarking \cite{ot4}) is worth mentioning. In the early work, secure multiparty computation \cite{tt2} and homomorphic encryption \cite{ot4} are proposed to generate watermarked data without seller's knowing the data, which are considered too expensive in practice \cite{ot1}. Then, some proposals leverage Oblivious Transfer (OT) \cite{np,otorigin} which is much more efficient in performance \cite{ot1,ot2,ot3}. Our scheme is inspired by these proposals, with two contributions: (1) there is no judge in our scheme; (2) we improve the cost and scalability for asymmetric watermarking.


% \noindent{\bf Comparison with previous work.}
We summarizes the comparison of Argus with previous work in Table \ref{tab:compare}. Column three and four (i.e. BSA and Custos) are two competitive solutions of Argus while column five to eight (AWM, ZKP, Hydra and Arbitrum) are primitives corresponding to $O(1)$-appeal, multi-period commitment and incentive model, respectively. Details are listed below:
\squishlist
\item{\bf\em Comparison with previous solutions.} Centralized schemes such as BSA \cite{bsa} can considerably disincentivize informers due to the opacity of payments. To increase the trust of payments, Custos \cite{custos} leverages blockchain. However, Custos does not consider strong accusation and cannot assess the severity of piracy, which is important in law enforcement. By contrast, Argus achieves full transparency along with all other properties. 
\item{\bf\em Comparison with state-of-the-art primitives:} 
\squishlistthree
\item Previous work of Asymmetric Watermarking (AWM) \cite{ot1,ot2,ot3,ot4} all rely on the existence of a ``trusted judge''. In addition, their appeal protocols introduce $O(N)$ bandwidth cost, which is unacceptable in blockchain scheme. 
\item Current Zero-Knowledge Proof (ZKP) \cite{zerocash,zkpcommit} can eliminate replay attack by enabling informers to prove their acquaintance of $id_{ij}$ without revealing the answer. However, current ZKP can introduce considerable performance overhead and gas consumption which limits system scalability. 
\item Commitment scheme (or so-called ``commit-reveal'') \cite{arbitrum} can address replay attack by dividing the single submission into phases of commitment and revealing, which is much more efficient than ZKP schemes. However, to fully evaluate piracy, the commitment phase should be relatively long, which delays owner's confirmation of piracy and informers' payments. 
\item  Sybil-proofness \cite{truebit,arbitrum} is introduced to disincentivize informers to report repeatedly: the more times a informer reports, the less bounty the informer can claim. However, existing sybil-proof incentive model merely depends on the total number of informers, which is known only when the collection period ends. 
\item By contrast, Argus overcomes the limitations of above primitives. In addition, further integration and optimization are introduced in this work.
 \squishlistthreeend

\squishlistend
%\squishlistoneone
%\item Centralized schemes such as BSA \cite{bsa} require detailed reports which contain the number of pirated copies, avenues, the identity of informers and other supporting evidence. informers are paid only when the reports are validated and directly induces settlement. However, as addressed before, the opacity and long process of payments can considerably disincentivize informers. 
%\item To increase the trust of payments, Custos \cite{custos} leverages blockchain by embedding private keys of different cryptocurrency accounts into watermark. Thus, guilty users are indicated if balances of corresponding accounts are withdrawn by informers. However, Custos does not consider the dispute of tracing and cannot evaluate piracy.
%\item Recent work of Asymmetric Watermarking (AWM) \cite{ot1,ot2,ot3,ot4} propose to leverage $1$-out-of-$N$ Oblivious Transfer~(OT) \cite{np} to obfuscate user's choice among $N$ versions of watermarked data. Thus, the probability of owner's successful frame-up is only $1/N$. However, informer is not supported and considered in these work. In addition, OT may introduce considerable bandwidth overhead especially when blockchain is leveraged.
%\item Zero-Knowledge Proof (ZKP) \cite{zerocash,zkpcommit} can eliminate replay attack by enabling informers to prove their acquaintance of bounty answer without revealing the answer. However, current ZKP can introduce considerable performance overhead which limits system scalability. 
%\item Commit scheme (or so-called ``commit-reveal'') \cite{arbitrum} can address replay attack by dividing the single submission into phases of commitment and revealing, which is much more efficient than ZKP schemes. However, to fully evaluate piracy, the commitment phase should be relatively long, which delays the revealing phase and informers' payments.
%\item Sybil-proof bounty \cite{truebit,arbitrum} is introduced to disincentivize informers to report repeatedly: the more times a informer reports, the less bounty the informer can claim. However, existing sybil-proof bounty merely depends on the total number of informers, which is ready only when the collection period ends. 
%\squishlistoneoneend



\section{Conclusions}

%Stopping piracy can protect the profits of copyright holders and the impetus of innovators. However, the covert propagation of pirated copies via Internet (cloud drive, BitTorrent, etc.) makes it challenging to discover, trace and quantify piracy, which delays copyright law enforcement and other mitigation actions. To address this challenge, piracy bounty is widely used to leverage the power of the crowd: bounty informers report piracy to copyright holders (or delegates) to claim bounties. Watermarking are sometimes used in the process to identify the source of piracy.
%However, in the real-world malicious settings, existing schemes of piracy bounty are either not incentive-compatible for reporting (e.g. nonpayments, de-anonymization) or not attack-resistant for tracing/quantifying (e.g. frame-up attack, sybil attack, replay attack).
%To circumvent drawbacks of existing work, we propose Argus, a novel piracy bounty framework for a wide range of traceable digital data types (e.g. media data and AI models) with technologies of blockchain, digital watermarking, cryptography and mechanism design. Our bounty scheme is transparent yet privacy-preserving and cheat-proof. Our optimized implementation is practical to work on public blockchains with very limited bandwidth.

Anti-piracy is fundamentally a procedure that relies on collecting  data from the open anonymous population, so how to incentivize credible reports is a question at the center of the problem. Academic researchers and real-world companies have come up with various incentive mechanisms. However, without explicitly prescribing the interests of different roles and the objectives of an anti-piracy system, designing such a mechanism has been more of a ``creative art'' than a systematic and disciplined exploration. Currently, there is no good framework to evaluate these designs and actual systems. 

The most essential value of our work is not the Argus system itself, but the approach leading to its design and implementation. We first state clearly the interests of different roles and the goal of full transparency without trusting any role. Once these are stated, all the design requirements naturally surface, such as Sybil-proofness, information-hiding submission, resistance to infringer's repudiation, etc; once these design requirements are clear, we are able to {\em deduce}, rather than {\em invent}, the general form of valid solutions; the deduced general form then boils down to a set of unavoidable technical obstacles, which we overcome by adapting crytopographic schemes, building contract code and optimizing performance. 

Argus exemplifies the outcome of this disciplined approach. It is superior to existing solutions in terms of the trust assumption and the assured properties. In particular, we draw the following conclusions: (1) it is feasible to build a fully transparent solution without introducing a trusted role. This could enable a paradigm shift for anti-piracy incentive solutions. Also, it is a compelling application scenario for public blockchains; (2) such a solution indeed consolidates all roles' interests fairly, i.e., as long as a role is not at fault, his/her interest will not be impaired by other malicious or at-fault roles; (3) besides logic soundness, the solution is economically practical, as a result of our effective optimizations.  





==> Argus SRDS Full/scalable.tex <==
\section{Making Argus Scalable}\label{sec:scalable}
As addressed in previous section, the scalability issue needs to be carefully considered especially when blockchain is leveraged. In this section, we will show how we optimize the onchain/offchain bandwidth consumption of Argus, which mainly leverages two technologies: state channel and private information retrieval, respectively.

\subsection{Optimizing Onchain bandwidth}
Given that typical blockchain (Bitcoin, Ethereum) can only handle $\sim$ 10 transactions per second and the process of OT involves multiple interactions/transactions, we leverage state channel technology to mitigate the overhead \cite{plasma,arbitrum}. Ideally, with state channel, transactions are only sent to chain at the start/end of data delivering. However, to support the whistleblowing process, corresponding $\{H(ID_i)\}$ should be public, which is considerably large per deal. Thus, we construct a Merkel tree style data structure to store $\{H(ID_i)\}$ offchain while leveraging the immutability of blockchain, which is illustrated in Figure \ref{fig:mt}. Every time, as soon as new trade occurs, the Merkel tree is updated along with only its root sent to the contract. And the rest of the Merkel tree can be kept offchain (e.g. in owner's bulletin board). 

% \begin{figure}[thbp]
% \fbox{
% \pseudocode{%
% \textbf{ Owner} \< \< \textbf{ User}  \\[0.1\baselineskip][\hline]
%  \<\< \\[-0.5\baselineskip]
% \{C_i\} \sample \ZZ_q \< \< \\
% r \sample \ZZ_q \< \< \\
%  R \gets r\cdot G \ \<\< \\
% \{C'_i\} \gets \{r \cdot C_i\}\\
%  \< \sendmessageright*{\{C_i\},R} \< 
% \pclb
%  \pcintertext[dotted]{Initializing Phase Ends} 
%   \<\< k \sample \ZZ_q \\
%  \<\< j \sample\set{1,\ldots,N} \\
%  \<\< PK_0 \gets C_j-k \cdot G \pclb
%  \pcintertext[dotted]{Choosing Phase Ends} 
%  \< \sendmessageleft*{PK_0} \< \\
%  PK'_0 \gets r\cdot PK_0 \ \<\< \\
%  r\cdot PK_i \gets C'_i-PK'_0 \<\< \\
%  \{E_i\} \gets \{H(r\cdot PK_i, R, i) \oplus M_i\} \<\<\\
%  \< \sendmessageright*{\{E_i\}} \< \pclb
%  \pcintertext[dotted]{Transferring Phase Ends} 
%  \<\< M_j = E_j \oplus H(k \cdot R, R, j) \\
%  }
%  }
%  \centering
% \caption{Zero-knowledge Whistleblowing with Trade Subtree} \label{fig:tradetree}
% \end{figure}

Since the whistleblower needs to prove his/her acquaintance of a valid $ID_i$ in a zero-knowledge style, the list of $\{ID_i\}$ should be obtained first by the whistleblower. However, direct querying the bulletin board exact $ID_i$ may leak the value of $ID_i$ to the owner. To mitigate the leakage, we embed additional bits in the ID called ``Trade-ID'', namely Watermarked ID is a catenation of a secret ID and a Trade-ID. once the whistleblower detects the Watermark ID, he or she should query the subtree corresponding to the Trade-ID and obtains the entire subtree. With the subtree, the whistleblower can then generate the two proofs:
\begin{enumerate}
    \item The detected secret ID is in a certain path of the subtree.
    \item There is a path traversing from the root of subtree to the root of the whole Merkel tree. 
\end{enumerate}

As illustrated in Figure \ref{fig:tradetree}, the first proof is required to be zero-knowledge to prevent leakage to owner while the second can be implemented using Merkel tree proof for better prover performance. Note that we catenate ${H(ID_i)}$ with index $i$ to facilitate the appealing process of users. As addressed in Section \ref{sec:zkw}, the whistleblower should send the proof along with an encryption of the answer to the contract. And the user can appeal to the contract that the decrypted answer is invalid via BLS signature. 
By contrast, for the structure in Figure \ref{fig:mt}, the whistleblower should send the encryption of ${H(ID_i)}||i$ to the contract and the user appeals as follows:
\begin{enumerate}
    \item The user decodes $H(ID'_i)$ and the index $i$ from the decryption of ${H(ID'_i)}||i$ and proves the correctness of the decoding with BLS signature. 
    \item The user proves that $i$-th leaf ${H(ID_i)}||i$ in the subtree conflicts with decoded $H(ID'_i)$ or conflicts with $PK_0$ during asymmetric watermarking. 
    \item If the ${H(ID'_i)}||i$ is incorrect in index $i$ but exists in subtree, the owner will be punished since the user is framed. 
\end{enumerate}
\begin{figure}[thbp]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/mt.pdf}
    \caption{The Merkel Tree for $H(ID)$ }
    \label{fig:mt}
\end{figure}
\subsection{Optimizing Offchain bandwidth}
The bandwidth overhead does not only exist for blockchain but also the offchain network. For asymmetric watermarking where $N=100$, compared to downloaded data size without protection, $100$ times of data size are transferred between the owner and the user \cite{}. In addition, the performance overhead of asymmetric encryption/decryption also burdens the owner/user. Therefore, we adapt the process of OT to mitigate the overhead of asymmetric encryption and introduce PIR to mitigate the bandwidth overhead:
\begin{enumerate}
    \item The owner encrypts $N$ copies of data using symmetric encryption (e.g. AES) with $N$ secret keys $\{K_i\}$, which is denoted as $\{Enc_{K_i}(D_i)\}$
    \item The user gets $K_j$ from $\{K_i\}$ via $1$-out-of-$N$ OT protocol.
    \item The user gets encrypted $Enc_{K_j}(D_j)$ from $\{Enc_{K_i}(D_i)\}$ via PIR protocol.
    \item The user decrypts $Enc_{K_j}(D_j)$ with $K_j$.
\end{enumerate}
For the bandwidth overhead, the above scheme can achieve the same security with a bandwidth consumption of $\Psi(|D|+N*|K|)$. Given that $|D|\gg |K|$, the bandwidth overhead is $\Psi(|D|)$ which approximates the data downloaded size without any protection. For the performance overhead, the symmetric encryption phase can be conducted offline and thus can be omitted. The performance of PIR is highly optimized by using Ring-LWE \cite{xpir}. The overhead of decrypting $Enc_{K_j}(D_j)$ is negligible compared to the network latency. The overhead of bandwidth and performance is evaluated in Section \ref{sec:eval}.


==> Argus SRDS Full/security.tex <==
% \subsection{Security Analysis}\label{sec:analysis}
% [* maybe we can move the detailed analysis to an appendix, and make this section a subsection inside Evaluation. We just need to say that (1) the appendix's model -- one owner, two licensees and two informers; (2) if a person has no fault, his interest will not be hurt even when others collude. -Shuo *]
% [* I haven't made a pass of this section. -Shuo *]
% As a blockchain-based solution, the referability of Argus is obvious. Thus, in this section, we focus on the security analysis of Argus from the perspective of completeness and soundness of Argus. with assumptions in Section \ref{sec:basicargus}.

% \begin{proposition}
% As long as piracy users are well informed about Argus and three assumptions hold, Argus satisfies the requirement of Completeness. 
% \end{proposition}
% \begin{remark}[Remark1]
% According to the watermark assumption, any piracy users obtain the data can detect the secret ID. According to the property of Sybil-proof bounty, the piracy users are incentivised to claim the blockchain-based bounty by reporting according to Section \ref{sec:spb}. The user cannot invalidate the report if he/she is guilty. And according to the blockchain assumption, any valid reports will be recorded onchain without censorship and cannot be altered in the future. \qed
% \end{remark}
% \begin{remark}[Remark2]
% The guilty user may launch {\em commitment contract} \cite{threat} to counteract the effects of Argus: if those piracy users do not report within a deadline $T'>T$, they will be better paid than that via the Argus contract. However, since $T$ in Argus is dynamically set, if there is no report, the $T$ will be extended automatically (Section \ref{sec:sbfproof}). Consequently, $T'$ has to be extended which disincentivises privacy users to follow the commitment contract.
% \end{remark}

% \begin{remark}[Remark3]
% The whistleblower may also cooperate via the commitment contract to sidestep the decrease of sybil-proof bounty: one can launch another contract to convince other whistleblowers to submit their answer to the commitment contract instead of the Argus contract. Then, the contract will redistribute bounty obtained from the Argus contract by deadline $T$. As long as the redistributed bounty is larger than that of participating Argus contract, the commitment contract can interfere the functionality of Argus contract. However, the contract encounters a similar dilemma of the commitment contract in Remark 1: as long as the reward in Argus contract exceeds that in the commitment contract, any whistleblower would still try Argus contract. In fact, to prevent possible sybil attack, the commitment contract should also leverage sybil-proof bounty. Since the total reward of commitment contract is less than that of Argus contract, the optimal choice for the whistleblowers not in the Argus contract should be submitting to both the Argus contract and the commitment contract, which does not affect the functionality of Argus contract.   
% % In Appendix \ref{sec:game}, we will prove that this leads to a Nash Equilibrium that except the whistleblowers already in the Argus contract, anyone followed would submit to both the Argus contract and the commitment contract.   
% \end{remark}

% \begin{proposition}
% As long as piracy users are informed about Argus and three assumptions hold, Argus satisfies the requirement of Soundness. 
% \end{proposition}
% \begin{remark}[Remark4]
% There are four possible scenarios to either incriminate the innocent user or exaggerate the number of piracy as follows, which are effectively mitigated in our design:
% \begin{itemize}
%     \item {Owner's frame-up.} Owner will not incriminate the innocent user because of the threat of heuristic asymmetric watermarking only if selfish assumption holds. 
%     \item {Whistleblower's frame-up.} Because of the randomness of user ID in the watermarked copy, the possibility of whistleblower's guessing the ID without watermarked copy is negligible. 
%     \item {Owner's over-report.} Because the whistleblower is submitting the ID in a zero-knowledge way. Thus, the owner cannot follow the whistleblower without knowing the piracy copy. In addition, with our design of punishment (Section \ref{sec:punishment}), the owner has no incentive to over-report since any whistleblowing is constrained by the sybil-proof bounty.
%     \item {Whistleblower's over-report.} With the selfish assumption and the design of anti-sybil bounty, the whistleblower will not resubmit the ID or redistribute the piracy to others. Anyone without the piracy cannot follow the whistleblower since the zero-knowledge style of submitting ID. \qed
% \end{itemize}
% \end{remark}

% \begin{remark}[Remark5]
% Above proof does not consider {\em owner's revenge} which is apparently irrational but might be long-term beneficial. Namely that the Owner may deliberately resubmit the ID to the contract as soon as the owner receives the privacy (either collected by himself/herself or even from colluded whistleblowers). The owner does not care about the bounty but the punishment to the pirates. However, as addressed previously, Argus is not the only source of evidence to identify the significance of piracy. Further forensics are required with the assistance of Argus \cite{anticollusion}.  
% \end{remark}

% \begin{proposition}
% The scalability improvement does not degrade the soundness, referability of Argus while the completeness is slightly affected. 
% \end{proposition}
% \begin{remark}[Remark6]
% It is obvious that state channel and storage compression do not affect above three metrics given adequate liveness and computation ability of counterparties. Similarly, using Merkel tree to reduce the onchain storage/bandwidth cost does not enable the owner/whistleblower to incriminate the innocent user. However, one possible impact to the t-completeness is that the owner might shut down the bulletin board to monopolize the reward for successful report, which in fact reduces the reported number of privacy. In fact, by doing this, the owner completely turns off the functionality of whistleblowing while the cost to collect piracy should be considerably increased. Considering the limitation of collecting piracy by owner himself/herself and the efficiency of whistleblowing, we believe that this is a rare case in reality. \qed   
% \end{remark}

==> Argus SRDS Full/trace.tex <==
\section{Guarding against infringer's repudiation}\label{sec:detect}


No role in Argus, even the owner, is assumed trusted. This presents a challenge: when the owner accuses a licensee for leaking a copy, the licensee can refute the accusation by arguing that the copy could have been leaked out by the owner himself. To resolve the dispute, Argus must make the evidence of the accusation so convincing that {\em the probability of the accused infringer being an innocent licensee is extremely small}. Hence, a true infringer's attempt to repudiate will be unsubstantiated.

%To approach the property, {\em asymmetric watermarking} (so-called buyer-seller watermarking \cite{ot4}) is proposed and investigated \cite{ot1,ot2,ot3}. The core idea of asymmetric watermarking is simple: by playing a certain protocol of data sharing, the licensee obtains an imperceptibly modified version of data which the owner does not know. Then, unless the owner gets a copy of the modified data, the owner can not frame the licensee with another version of data.
%
%In early work, secure multiparty computation \cite{tt2} and homomorphic encryption \cite{ot4} are proposed to generate watermarked data without seller's knowing the data, which are considered too expensive in practice \cite{ot1}. Consequently, the state-of-the-art work leverage Oblivious Transfer (OT) \cite{np,otorigin} which is much more efficient in performance \cite{ot1,ot2,ot3}: the seller generates $N$ copies of data watermarked with different unique IDs and plays OT protocol with the buyer. Then, the licensee can obtain only one copy without owner's knowing which one. Thus, when there is a dispute, the seller and the buyer can refer to a {\em judge} providing related evidence. In Section \ref{sec:detect}, we will further improve asymmetric watermarking in cost/scalability.


To approach the objective, we use a $1$-out-of-$N$ Oblivious Transfer (OT) \cite{np,otorigin} protocol to achieve this goal. The $1$-out-of-$N$ OT protocols were used for data sharing \cite{ot1,ot2,ot3,ot4}: the owner generates $N$ different copies of data (e.g. via watermarking) and plays OT protocol with the licensee. Then, the licensee can obtain only one copy without owner's knowing which one. Thus, owner can infer the chosen version with a pirated copy.  When there is a dispute between a licensee and the owner, they can submit messages occurred in OT to a {\em trusted judge} for resolving disputes. There is only a $\frac{1}{N}$ probability that the successfully accused licensee is innocent. 

A goal of Argus is not to have any trusted role, so the Argus contract has to implement the functionalities of the ``judge'' on a public blockchain. However, this may introduce a big bandwidth overhead: messages incurred in OT are proportional to $O(N)$. To achieve a desirable security level with a large $N$ (e.g. $10,000$), existing solutions introduce enormous on-chain overhead (e.g. bandwidth, execution, storage). 

To greatly reduce the overhead, we introduce {\em $O(1)$-Appeal} which only incurs $O(1)$ on-chain messages and operations. $O(1)$-Appeal has two properties:
\squishlistoneone
\item {\bf Obliviousness}. It is the property of $1$-out-of-$N$ OT \cite{np,otorigin}: (1) the licensee can arbitrarily choose and obtain $1$ data from $N$ candidate data but cannot know the unchosen data; (2) the owner does not know which data are chosen by the licensee. This property guarantees that the probability to successfully incriminate an innocent licensee is $\frac{1}{N}$ and thus an infringer is hard to deny accusation with a large $N$ (e.g. $10000$). 
\item {\bf Non-repudiation}. When the licensee is accused, the licensee can appeal by showing committed records. When there is a dispute, neither the owner nor licensees can deny which copy the licensee had chosen in the previous OT protocol. The contract is able to give a conclusive answer.
\squishlistoneoneend

\subsection{Constant-Size-OTRecord Appeal ($O(1)$-Appeal)}
% [*add subsection here -shuo Constant-Size-OTRecord Appeal, a.k.a. O(1)-Appeal*]

The protocol of $O(1)$-Appeal is shown in Figure \ref{fig:ot}, which includes four sub protocols: $\mathsf{Initilize}$, $\mathsf{GenerateEvidence}$, $\mathsf{TransferData}$, $\mathsf{Appeal}$. The first three sub protocols are very similar\footnote{The only difference is that we add a step (step 2) in $\mathsf{GenerateEvidence}$.} to those in \cite{np}, while the fourth sub protocol is our new invention that incurs only an $O(1)$ on-chain cost. Unlike in Section \ref{sec:basicargus}, the owner does not have to commit OTEvidence (i.e. $R$) to the contract. Instead, $R$ can be signed and kept locally.
For simplicity, we assume that the owner and the licensee do not abort during the procedure (e.g. this can be ensured by using the state channel technology \cite{plasma} or the fair exchange protocol \cite{fairswap}). 

\begin{figure}[]
\begin{center}
\fbox{
\procedure[syntaxhighlight=false,mode=text,width=0.44\textwidth,codesize=\footnotesize]{OT with $O(1)$-Appeal}{
\squishlist
\vspace{5pt}
  \item {\bf Public parameters:} field $\ZZ_q$, generator $G \in \mathbb{G}$  
  \item{\bf Owner input:} $N$ versions of data $\set{D_i} (i=1,\ldots,N)$, Owner's private key $sk^O$ 
  \item {\bf Licensee input:}  Licensee's private key $sk^L$  
  \item {\bf Sub Protocols}:
  \squishlistthreeone
  \item {$\mathsf{OT.Initialize}$:} 
  \squishlisttwo
  \item Owner randomly generates and signs $N$ elements $\set{P_1, \ldots, P_N} \in \mathbb{G}^N $ and samples a random number $s \in \ZZ_q$. 
  \item Owner publishes $a_s=s\cdot G$, $\set{P_i}$ and keeps $\{P'_i\}\gets\{s \cdot P_i\} (i=1,\ldots,N)$ locally. 
  \item Licensee samples and keeps two secrets $r \in \ZZ_q$, $l \in [N]$. 
  \squishlisttwoend
  \item {$\mathsf{OT.GenerateEvidence}$:}
    \squishlisttwo
   \item Licensee signs and sends $R = P_l- r \cdot G$ to Owner. 
   \item Owner signs and sends $\sig_{sk^O}(\sig_{sk^L}(R))$ to Licensee.
   \squishlisttwoend
  \item {$\mathsf{OT.TransferData}$:} 
  \squishlisttwo
   \item Owner computes $R' \gets s\cdot R$, $Q_i \gets P'_i-R'$ and sends $\{E_i\} \gets \{\mathcal{H}(Q_i, a_s, i) \oplus D_i\} (i=1,\ldots,N)$ to Licensee. 
   \item Licensee gets $D_l= E_l \oplus \mathcal{H}(r \cdot a_s, a_s, l)$.
   \squishlisttwoend
  \item {$\mathsf{Appeal}$:} 
  \squishlisttwo
   \item Licensee being accused of leaking $D_{l_x}$ can send a tuple $(\sig_{\ast}(R)$, $r$, $l)$ to contract $\mathcal{C}$ (i.e. judge), where $\sig_\ast(R)$ is signed by both Owner and Licensee. 
   \item $\mathcal{C}$ verifies if $P_l - r \cdot G=R$ and $l \neq l_x$. If yes, Licensee is falsely accused. Otherwise the appeal fails.
   \squishlisttwoend
\squishlistthreeoneend
\squishlistend
}
}
\end{center}
\vspace{-10pt}
\caption{Licensee gets one data $D_l$ from $N$ data $\set{D_1,\ldots,D_N}$ from Owner via $O(1)$-Appeal with $OTEvidence=R$ and $OTRecord=(r,l)$.} \label{fig:ot}
\vspace{-20pt}
\end{figure}

Different from previous work that utilizes transferred vectors (e.g. $\set{E_1,\ldots,E_N}$) in $\mathsf{TransferData}$ for dispute resolving, we find that utilizing one transferred variable $R$ in $\mathsf{GenerateEvidence}$ can be of the same effect. Our key discovery is that $R$ has a one-to-one correspondence to the licensee's chosen index $l$ (see Theorem \ref{th:7}). Therefore, $R$ can be used as the evidence to indicate the licensee's chosen index in the dispute-resolving stage (i.e. the appeal stage). 

As shown in $\mathsf{Appeal}$ in Figure \ref{fig:ot}, if $R$ is signed by owner/licensee and indicates that the corresponding index $l$ differs from accused index $l_x$, we can conclude that the licensee is wrongly accused. We prove the Obliviousness and Non-repudiation of OT with $O(1)$-Appeal in Appendix \ref{sec:appealsecurity}.

Though $O(1)$-Appeal has greatly reduced the on-chain overhead of the appeal stage, there is still a considerable cost of the off-chain bandwidth in $\mathsf{TransferData}$. To reduce the off-chain bandwidth overhead, in Section \ref{sec:construct}, we will further leverage a PIR protocol \cite{xpir} and slightly adapt $O(1)$-Appeal, which guarantees that the size of the data transferred is about the size of data $D_l$. In addition, we will show how to integrate $O(1)$-Appeal with the information-hiding report scheme in Appendix \ref{sec:bigpic}.







==> Argus SRDS Full/zkp.tex <==
\section{Information Hiding for Report Submission} \label{sec:zkw}
As mentioned in the introduction, full transparency is a major advancement of Argus. To achieve it, our design requires an effective strategy for information hiding. Specifically for the procedure of report submission, Argus needs to ensure that, although everybody in the open population can see the interactions between an informer and the Argus contract, nobody other than the informer can replay the interactions effectively. (Note that the informer himself will not replay due to the Sybil-proof property of the incentive model discussed in Section \ref{sec:quantify}.) 

\subsection {The objectives of the information-hiding submission} \label{sec:zkpobj}

Before designing the information-hiding submission procedure, we first consider the interests of different roles, and specify the objectives to be achieved:

\squishlistoneone
\item First, the owner's interest is to get an accurate count of the number of piracy copies. The count should not be inflated, meaning that no replay attack as described above should be possible.
\item Second, the owner wants to run a bounty campaign for a long duration, e.g., 3-6 months, so that the magnitude of the piracy infringement can be evaluated more thoroughly. However, an informer's interest is to get a timely payout after a report is submitted successfully.
\item Third, both the owner and the informers want the submission to be concluded in a short period of time. Also, the submission should be efficient. Since Argus runs on a public blockchain, the gas consumption of the procedure is required to be very low.
\squishlistoneoneend

\subsection {Previous proposals and their limitations}
Previous work have proposed commitment scheme \cite{hydra,commitment} and zero-knowledge proof \cite{zkbounty,arbitrum} to eliminate the replay attack. However, in Argus's scenarios, they may either conflict with the interests of owner/informer or encounter serious performance problems:
\squishlistoneone
\item In traditional commitment scheme, the informer submits a commitment of the report (e.g. Hash) in the first period (``commitment phase'') and reveals the report during a following period (``reveal phase'').  Informers' reports are not accepted in the second phase unless a corresponding commitment exists in the first phase. Therefore, the replay attack cannot succeed since the attacker cannot generate valid commitments in the first phase. However, setting the length of the commitment phase has a dilemma because of the different interests of the owner and the informers (definitions in Section \ref{sec:zkpobj}): (1) if the phase is too long, it is not timely for the owner to validate infringers and take subsequent actions, and the informer needs to wait for a long time to get the bounty; (2) if it is too short, the number of the reported pirated copies cannot accurately reflect the severity of the infringement. 
\item In a zero-knowledge proof (ZKP) scheme, the informer can generate a proof to show the possession of a pirated copy. In the ZKP scheme, the bounty can be paid as soon as the contract verifies the proof, which is what we desire. However, the ZKP scheme has a prohibitively high performance overhead and gas cost (see Section \ref{sec:eval}).  
\squishlistoneoneend

\subsection {Multi-period Commitment Scheme}
% [* Please change to multi-period commitment scheme. -Shuo *]
To achieve the objectives with good performance, we propose a novel technique called multi-period commitment. The scheme can be considered as an extension of the traditional commitment scheme, but has a good performance. Meanwhile, it has the advantage similar to the zero-knowledge proof --- the owner can still set a long bounty campaign period, but confirm every report almost in real time. 

Our scheme allows multiple commit-and-reveal phases so that there are sufficient time windows for the informers to submit piracy reports. For a desired length of collection period $T$, the owner can divide $T$ into $K$ {\bf\em sub-periods} $\set{T_1,\ldots,T_K}$. Each sub-period $T_i \quad (1<i<K)$ is the $i$-th commitment phase and also the $(i-1)$-th reveal phase. In other words, an informer can claim a bounty in $T_{i+1}$ ($i$-th reveal phase) by revealing if the corresponding commitment is submitted in $T_{i}$ ($i$-th commitment phase). 

However, dividing into periods introduces a problem: informers can replay the process of commit-reveal in sub-periods $T_i$ and $T_{i+1}$ to later sub-periods $T_j$ and $T_{j+1} \quad (j>i)$. To defend again this kind of replay attack, we introduce a time stamp into the formula of commitment and process of verification: if we denote the piracy report as $X$ and hash function as $\mathcal{H}$, and there is a predefined list $L[\cdot]=\set{\mathcal{H(H(}X||1)),\ldots,\mathcal{H(H(}X||K))}$ in the contract. Then, the commitment $cm$ submitted in $T_i$ can be $\mathcal{H(H(}X||i)||n)$ where ``$||$'' denotes concatenation and ``$n$'' denotes a randomized nonce. In corresponding reveal phase $T_{i+1}$, $rv=\mathcal{H}(X||i)$ and $n$ should be submitted to the contract for verification that $\mathcal{H(}rv||n)=cm$ and $\mathcal{H(}rv)=L[i]$. By this reinforcement, the aforementioned replay attack cannot pass the verification ``$\mathcal{H(}rv)=L[j]$'' in later sub-periods $T_{j+1} \quad (j>i)$.

The multi-period commitment scheme achieves the objectives given in Section \ref{sec:zkpobj}:
\squishlistoneone
    \item The multi-period commitment scheme foils the replay attack, thus meets the first objective.
    \item The multi-period commitment scheme supports an arbitrary length of collection period $T$, thus meets the second objective.
    \item With a sufficiently large $K$, each sub-period can be short enough\footnote{We will show the storage overhead of setting a large $K$ in Appendix \ref{sec:imple}.}. Thus, informers can reveal reports and get their rewards within a short interval after commitments. The owner gets quick confirmations of the infringers. This achieves the third objective.
%    \item Time-varying commitment scheme does not leverage expensive cryptographic operations such as bilinear paring \cite{bn254}, thus demonstrate an superior performance/cost compared to ZKP scheme (details in Section \ref{sec:eval}). In other words, the fouth objective is also satisfied. 
\squishlistoneoneend
% One critical issue of naive Argus is that any report is public, which causes three aspects of challenges:
% \begin{enumerate}
% \item Anyone can follow the previous report to send the same unique ID, which breaks the soundness.
% \item Nodes of the blockchain may launch front-running attack \cite{teether} after the transaction of informer is broadcasted, which is unfair to the informer. 
% \item From the report, the owner can infer the index of the watermarked data chosen by the user. Then, the owner may incriminate or even revenge the guilty user with enormous report.
% %\item The guilty user may incriminate himself/herself to threat informers not  
% \end{enumerate}

%Optimal ate pairing over Barreto-Naehrig (BN) curve.

% Previous work have proposed using {\em commit-and-reveal} to address the first two challenges: the informer commits $Hash(ID||addr)$ (``$||$'' denotes concatenation) to the contract in the first phase and then reveal the ID in the second phase \cite{}. However, commit-and-reveal solutions cannot address the third challenge since the owner still acquires from the ID which data the user chose. Moreover, to provide a long-time protection of the data, the length of the first phase should be neither not too short nor too long. If too long, the ID is not timely revealed and validated which deters consequent actions (e.g. forensics, judgments); If too short, the data are not protected afterwards which is not desired.
% In Appendix \ref{sec:}, we will show that using multiple rounds of commit-and-reveal is inefficient in blockchain. 

% Therefore, we leverage Zero-knowledge Proof to eliminate previous three challenges. For every informer, ID is obtained after watermark detection. Then, the informer should send following data to the contract:
% {\em
% Given input $\{Hash(ID_i)\}$ and the informer's $addr$, output $cm$, informer makes  ZK proof that ``I know the value of ID which satisfies $Hash(ID) \in \{Hash(ID_i)\}$, and the output $cm=Hash(ID||addr)$''
% }

% With the $\{Hash(ID_i)\}$ in the contract already deployed in asymmetric watermarking, the informer only needs to send $cm$ and corresponding ZK proof to the contract, which contains ZK verification logic. It is straight-forward that above three challenges are addressed. 

% However, merely using ZK proof leaves a vulnerability that the owner may incriminate innocent users without revealing anything, which disables the appealing of users. Therefore, besides the ZK proof, we need another mechanism to ensure the user can appeal while three above challenges are still addressed. To achieve this, we propose using a derived form of BLS signature \cite{bls} described as follows (details in Figure \ref{fig:zkw}):
% \begin{enumerate}
% \item The user generates a secret key $k$ and calculates $K=kG_1$. Then, $K$ is published as the public key.
% \item The informer generates a secret number $r$ and a tuple $(T=ID' \oplus rK, R=rG_2)$. ``$\oplus$'' is a XOR-like operations defined in \cite{}. Then, the tuple is sent to the contract along with previous ZK proof.
% \item The contract verifies the ZK proof. If validated, the user can choose to appeal by providing that the decryption of the tuple is incorrect: 
% \begin{enumerate}
% \item The user calculates $D=rK$ using $k$ and $R$ (i.e. $D=kR$).
% \item The user sends $D$ to the contract which performs verification by $\hat e(D, G_2) = \hat e(K,R)$ where $\hat e(\cdot,\cdot)$ denotes a bilinear pairing operation \cite{bn256}.
% \item If verification passes, the contract calculates $T \oplus D = ID' $ and verifies that: (i) $Hash(ID') \not\in \{Hash(ID_i)\}$ which indicates the tuple is false or (ii) $Hash(ID')$ conflicts with $PK_0$ which indicates a frame-up. 
% \item If case (i) occurs, corresponding report will be marked invalid and the user will not be punished. If case (ii) occurs, the owner will be punished while the user is compensated with considerable reward.
% \end{enumerate}
% \end{enumerate}

==> pre.tex <==
\section{Preliminaries}\label{sec:pre}
\subsection{Primitives}
{\em Secure watermarking}\cite{image,audio,software,dnnwatermark}. For simplicity, we formulate the digital watermarking system as a tuple $(x, y, id, E_W, D_W)$, where ${x, y, id, E_W, D_W}$ denotes original/watermarked data, embedded ID, watermark embedding/detection algorithm, respectively. They have the following relationship: $ y = E_W (x, id), id = D_W (y)$. Two important features of secure watermarking are {\em robustness} (even if $y$ is considerably modified as $y'$,  $D_W (y')$ still equals $id$) and {\em security} ($D_W$ can conceal relevant information to prevent attackers from directly removing watermark).

Unfortunately, even if a buyer is traced and incriminated via watermark detection results, the user may deny the guilt or significance of piracy since the seller and third-parties can also redistribute the watermarked data leading to a frame-up or an overestimate. Consequently, the disputes may stagger later copyright enforcement unless further evidence is provided.   

To address the dispute, {\em asymmetric watermarking} (so-called buyer-seller watermarking \cite{ot4}) is proposed and investigated \cite{ot1,ot2,ot3}. In early work, secure multiparty computation \cite{tt2} and homomorphic encryption \cite{ot4} are proposed to generate watermarked data without seller's knowing the data, which are considered too expensive in practice \cite{ot1}. Consequently, state-of-the-art work leverage Oblivious Transfer (OT) \cite{np,otorigin} which is much more efficient in performance \cite{ot1,ot2,ot3}: the seller generates $N$ copies of data watermarked with different unique IDs and plays OT protocol with the buyer. Then, the user can obtain only one copy without owner's knowing which one. Thus, when there is a dispute, the seller and the buyer can refer to a {\em judge} providing related evidence. In Section \ref{sec:detect}, we will further improve asymmetric watermarking in cost/scalability.
\subsection{Blockchain}
Blockchain is a distributed ledger system running on nodes among a P2P network. With the combination of consensus protocol and cryptography, nodes can execute programs with a same logic to reach consensus about the ledger states without trusting each other. In the P2P network, nodes send or propagate signed transactions to or from other nodes. Moreover, nodes are supposed to record and validate every transaction in order to ensure the correctness of its local ledger. When divergence occurs, consensus protocol functions, such as proof-of-work (POW) \cite{bitcoin}, proof-of-stake (POS) \cite{mauve}, PBFT \cite{pbft} and Raft\cite{raft}. 
%Above protocols all depend on ``votes'' from the distributed nodes while ``votes'' vary in forms for different consensus protocols. 

%The form of the vote highly relates to the type of the blockchain. In {\em public blockchain} such as Bitcoin \cite{bitcoin} and Ethereum \cite{ethereum}, every node is free to vote. Thus, in order to mitigate the risk of Sybil attack \cite{pbft}, computation power (i.e. POW \cite{bitcoin}) or stake (i.e. POS \cite{mauve}) is required to increase the cost of vote. By contrast, in {\em permitted blockchain}, such as Hyperledger \cite{hyperledger} and Corda \cite{corda}, only permitted node can vote. With this constraint, PBFT is enough to guarantee the consistency of blockchain data. With additional conditions, Raft can be used \cite{coco}. As a consequence, permitted blockchain is considered to be more efficient in performance with less decentralization compared with public blockchain. 

%which is first proposed by Satoshi Nakamoto in 2009 \cite{bitcoin}. 
%With the combination of consensus protocol and cryptography, nodes can execute programs with a same logic to reach consensus about the ledger states without trusting each other. In the P2P network, nodes can send or propagate signed transactions to or from other nodes. Moreover, nodes are supposed to record and validate every transaction in order to ensure the correctness of its local ledger. When divergence occurs, consensus protocol functions, such as proof-of-work (POW) \cite{bitcoin}, proof-of-stake (POS) \cite{mauve}, PBFT \cite{pbft}, Raft\cite{raft}. Above protocols all depend on ``votes'' from the distributed nodes while ``votes'' vary in forms in different consensus protocols. 
%
%The form of the vote depends on the type of the blockchain. In public blockchain such as Bitcoin and Ethereum, every node is free to vote. Thus, in order to mitigate the risk of Sybil attack \cite{pbft}, computation power (i.e. POW \cite{bitcoin}) or stake (i.e. POS \cite{mauve}) is required to increase the cost of vote. By contrast, in permitted blockchain, such as Hyperledger \cite{hyperledger} and Corda \cite{corda}, only permitted node can vote. With this constraint, PBFT is enough to guarantee the consistency of blockchain data. With additional conditions, Raft can be used \cite{coco}.

The above mechanisms lead to one most important feature of blockchain system called {\em decentralization}, which means the ledger is not secured by a centralized authority but distributed nodes. To extend the forms of decentralized trust and facilitate complicated applications over blockchain, script system \cite{bitcoin} or smart contracts \cite{ethereum} are introduced to support functionalities such as freezing/unfreezing funds, time-stamping, etc. These functionalities further enable a variety of applications which requires high confidence of trust, such as blockchain-based bounty system. 

Bounty systems have been demonstrated efficient in various scenarios such as program bug \cite{}, software piracy \cite{}, etc. However, the uncertainty of risking nonpayments can considerably undermine third-parties' incentives of cooperation. As a result, blockchain-based bounty mechanism are widely proposed with enforcement of rewarding, which is similar to that of blockchain-based exchange protocol \cite{fairswap}.

For example, to collect the watermarked data for detection, it is believed that the seller should cooperate with bounty hunter to circumvent technical obstacles \cite{presentation,custos}. Custos \cite{custos}, which is most related to our work, has proposed to design watermarked information as the private keys of different cryptocurrency accounts with balance. Consequently, any well-informed piracy users would extract the information to obtain certain accounts' balance, which leads to an on-chain transaction. The transaction can indicate corresponding illegal buyers and serve as evidence for further forensics and judgments. In summary, the blockchain-based incentive mechanism has enabled a credible threat to deter users from redistributing pirated copies. Similarly, Veredictum \cite{veredictum} has proposed to incentivise third-parties as crawlers for piracy copies through a bounty contract \footnote{According to Veredictum's latest whitepaper, current implementation does not leverage watermark \cite{Veredictumpaper}.}. 

Blockchain-based bounty is also leveraged in other scenarios. For example, Hydra \cite{hydra} has proposed to attract experienced hackers to submit bugs of valuable contract via blockchain-based bounty. They also propose commit-and-reveal with submarine commitment to mitigate front-running attack in blockchain. Arbitrum \cite{arbitrum} has proposed an efficient trusted off-chain computation mechanism based on the supervision of third-parties incentivized by blockchain-based bounty.
\subsection{Sybil attack}
Incentive mechanism
\subsection{Related Cryptographic Primitives}
In this section, we briefly introduce three cryptographic primitives involved in Argus: Oblivious Transfer and Private Information Retrieval.
\subsubsection{Oblivious Transfer} 
A $K$-out-of-$N$ Oblivious Transfer (OT) between an owner and an user is a cryptography protocol which guarantees following two properties:
\begin{itemize}
\item The user can arbitrarily choose $K$ data to obtain from $N$ candidate data. The user cannot know the unchosen data.
\item The owner cannot know which $K$ data are chosen by the user.
\end{itemize}

\begin{figure*}[thbp]
\fbox{
\pseudocode{%
\textbf{ Owner} \< \< \textbf{ User}  \\[0.1\baselineskip][\hline]
 \<\< \\[-0.5\baselineskip]
\{C_i\} \sample \ZZ_q \< \< \\
r \sample \ZZ_q \< \< \\
 R \gets r\cdot G \ \<\< \\
\{C'_i\} \gets \{r \cdot C_i\}\\
 \< \sendmessageright*{\{C_i\},R} \< 
\pclb
 \pcintertext[dotted]{Initializing Phase Ends} 
  \<\< k \sample \ZZ_q \\
 \<\< j \sample\set{1,\ldots,N} \\
 \<\< PK_0 \gets C_j-k \cdot G \pclb
 \pcintertext[dotted]{Choosing Phase Ends} 
 \< \sendmessageleft*{PK_0} \< \\
 PK'_0 \gets r\cdot PK_0 \ \<\< \\
 r\cdot PK_i \gets C'_i-PK'_0 \<\< \\
 \{E_i\} \gets \{H(r\cdot PK_i, R, i) \oplus M_i\} \<\<\\
 \< \sendmessageright*{\{E_i\}} \< \pclb
 \pcintertext[dotted]{Transferring Phase Ends} 
 \<\< M_j = E_j \oplus H(k \cdot R, R, j) \\
 }
 }
 \centering
\caption{Basic OT \cite{np}} \label{fig:ot}
\end{figure*}



OT have many implementations and optimizations \cite{ote,np,otorigin,simple}. Without loss of generality, we adopt Naor-Pinkas $1$-out-of-$N$ protocol in this work \cite{np}, which is illustrated in Figure \ref{fig:ot}:
%$N$ messages $M_1,M_2,\dots,M_N$
\begin{enumerate}
\item {\bf Initialize .} The owner generates $N$ random points $ \{C_i \in  Z_q\} (1\le i \le N)$ and a random number $r$. Then, $ \{C_{i} \}$ and $R=r\cdot G$ are published. The owner also precomputes $\{r \cdot C_{i} \}$.
\item {\bf Choose.} The user chooses a random number $k$ and an arbitrary index $j$ within $\{1,2,\dots,N\}$. Then, the user calculates $PK_0=C_j-k\cdot G$ which is then sent to the owner. 
%and records $PK_0$ in the contract.
\item {\bf Transfer.} The owner calculates $r \cdot PK_0$ and calculate $r\cdot PK_i=r\cdot C_{i}-r \cdot PK_0$ with precomputed $\{r \cdot C_{i} \}$. Then, $\{H(r\cdot PK_i, R, i) \oplus M_i\}$ are sent to the user. Since the user can calculate $k \cdot R$ which equals $r\cdot PK_j$, the user can obtain chosen data $M_j = (H(r\cdot PK_j, R, j) \oplus M_j) \oplus H(k \cdot R, R, j) $.
\end{enumerate}




% \subsubsection{Zero-knowledge Proof}
% Zero-knowledge proof (ZKP) is a cryptography protocol used in various systems \cite{zerocash,arbitrum,hawk}. ZKP can be represented by a tuple $(P,V,a,w)$ where $P/V$ denotes proving programs/verifying programs and $a/w$ denotes public input/secret witness of the prover. ZKP should have following three properties:   
% \begin{itemize}
% \item {\bf Completeness.} If the prover knows $w$, then the prover can generate a proof which can be validated by the verifier: $Pr[V(a,P(a,w))=0] = negl(\lambda) \label{eq:zkp}$
% \item {\bf Soundness.} If the prover does not know $w$, then the prover cannot generate a valid proof with a fake $w'$: $Pr[V(a,P(a,w'))=1] = negl(\lambda) \label{eq:zkp}$
% \item {\bf Zero-knowledge.} The verifier cannot learn anything from the proof of the prover.
% \end{itemize}

% $P/V$ can be either interactive \cite{interactive} or non-interactive \cite{zksnark}. And state-of-the-art ZKP introduce an another powerful property called {\em succinctness}. ZKP with succinctness, such as zk-SNARK \cite{zksnark}, can generate a fixed-length proof in bytes for arbitrary programs, which enables enormous scenarios and applications. In Section \ref{sec:zkw}, we will leverage ZKP to protect whistleblowers' report from being copied by others.
% %zk-SNARK to generate the binary of prover's program with verifier's logic in the contract.

\subsubsection{Private Information Retrieval}
Private Information Retrieval (PIR) is similar to Oblivious transfer except that in PIR the user is allowed to obtain all candidate data. The optimization goal of PIR is that the user can obtain intended data with negligible computation/communication overhead of both sides of owner/user. Various implementations of PIR have been shown \cite{xpir} and state-of-the-art PIR scheme are based on homomorphic encryption \cite{pir1,pir}. As one of state-of-the-art work, XPIR leverages Ring-LWE encryptions \cite{ring} and have demonstrated sufficient performance \cite{xpir}. To mitigate the bandwidth problem in asymmetric watermarking, we will use XPIR as a stand-along module in Section \ref{sec:imple} and thus do not introduce XPIR's details. \footnote{For details of XPIR, please refer to \cite{xpir} and code repo \cite{xpirrepo}}. 

==> scalable.tex <==
\section{Making Argus Scalable}\label{sec:scalable}
As addressed in previous section, the scalability issue needs to be carefully considered especially when blockchain is leveraged. In this section, we will show how we optimize the onchain/offchain bandwidth consumption of Argus, which mainly leverages two technologies: state channel and private information retrieval, respectively.

\subsection{Optimizing Onchain bandwidth}
Given that typical blockchain (Bitcoin, Ethereum) can only handle $\sim$ 10 transactions per second and the process of OT involves multiple interactions/transactions, we leverage state channel technology to mitigate the overhead \cite{plasma,arbitrum}. Ideally, with state channel, transactions are only sent to chain at the start/end of data delivering. However, to support the whistleblowing process, corresponding $\{H(ID_i)\}$ should be public, which is considerably large per deal. Thus, we construct a Merkel tree style data structure to store $\{H(ID_i)\}$ offchain while leveraging the immutability of blockchain, which is illustrated in Figure \ref{fig:mt}. Every time, as soon as new trade occurs, the Merkel tree is updated along with only its root sent to the contract. And the rest of the Merkel tree can be kept offchain (e.g. in owner's bulletin board). 

% \begin{figure}[thbp]
% \fbox{
% \pseudocode{%
% \textbf{ Owner} \< \< \textbf{ User}  \\[0.1\baselineskip][\hline]
%  \<\< \\[-0.5\baselineskip]
% \{C_i\} \sample \ZZ_q \< \< \\
% r \sample \ZZ_q \< \< \\
%  R \gets r\cdot G \ \<\< \\
% \{C'_i\} \gets \{r \cdot C_i\}\\
%  \< \sendmessageright*{\{C_i\},R} \< 
% \pclb
%  \pcintertext[dotted]{Initializing Phase Ends} 
%   \<\< k \sample \ZZ_q \\
%  \<\< j \sample\set{1,\ldots,N} \\
%  \<\< PK_0 \gets C_j-k \cdot G \pclb
%  \pcintertext[dotted]{Choosing Phase Ends} 
%  \< \sendmessageleft*{PK_0} \< \\
%  PK'_0 \gets r\cdot PK_0 \ \<\< \\
%  r\cdot PK_i \gets C'_i-PK'_0 \<\< \\
%  \{E_i\} \gets \{H(r\cdot PK_i, R, i) \oplus M_i\} \<\<\\
%  \< \sendmessageright*{\{E_i\}} \< \pclb
%  \pcintertext[dotted]{Transferring Phase Ends} 
%  \<\< M_j = E_j \oplus H(k \cdot R, R, j) \\
%  }
%  }
%  \centering
% \caption{Zero-knowledge Whistleblowing with Trade Subtree} \label{fig:tradetree}
% \end{figure}

Since the whistleblower needs to prove his/her acquaintance of a valid $ID_i$ in a zero-knowledge style, the list of $\{ID_i\}$ should be obtained first by the whistleblower. However, direct querying the bulletin board exact $ID_i$ may leak the value of $ID_i$ to the owner. To mitigate the leakage, we embed additional bits in the ID called ``Trade-ID'', namely Watermarked ID is a catenation of a secret ID and a Trade-ID. once the whistleblower detects the Watermark ID, he or she should query the subtree corresponding to the Trade-ID and obtains the entire subtree. With the subtree, the whistleblower can then generate the two proofs:
\begin{enumerate}
    \item The detected secret ID is in a certain path of the subtree.
    \item There is a path traversing from the root of subtree to the root of the whole Merkel tree. 
\end{enumerate}

As illustrated in Figure \ref{fig:tradetree}, the first proof is required to be zero-knowledge to prevent leakage to owner while the second can be implemented using Merkel tree proof for better prover performance. Note that we catenate ${H(ID_i)}$ with index $i$ to facilitate the appealing process of users. As addressed in Section \ref{sec:zkw}, the whistleblower should send the proof along with an encryption of the answer to the contract. And the user can appeal to the contract that the decrypted answer is invalid via BLS signature. 
By contrast, for the structure in Figure \ref{fig:mt}, the whistleblower should send the encryption of ${H(ID_i)}||i$ to the contract and the user appeals as follows:
\begin{enumerate}
    \item The user decodes $H(ID'_i)$ and the index $i$ from the decryption of ${H(ID'_i)}||i$ and proves the correctness of the decoding with BLS signature. 
    \item The user proves that $i$-th leaf ${H(ID_i)}||i$ in the subtree conflicts with decoded $H(ID'_i)$ or conflicts with $PK_0$ during asymmetric watermarking. 
    \item If the ${H(ID'_i)}||i$ is incorrect in index $i$ but exists in subtree, the owner will be punished since the user is framed. 
\end{enumerate}
\begin{figure}[thbp]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/mt.pdf}
    \caption{The Merkel Tree for $H(ID)$ }
    \label{fig:mt}
\end{figure}
\subsection{Optimizing Offchain bandwidth}
The bandwidth overhead does not only exist for blockchain but also the offchain network. For asymmetric watermarking where $N=100$, compared to downloaded data size without protection, $100$ times of data size are transferred between the owner and the user \cite{}. In addition, the performance overhead of asymmetric encryption/decryption also burdens the owner/user. Therefore, we adapt the process of OT to mitigate the overhead of asymmetric encryption and introduce PIR to mitigate the bandwidth overhead:
\begin{enumerate}
    \item The owner encrypts $N$ copies of data using symmetric encryption (e.g. AES) with $N$ secret keys $\{K_i\}$, which is denoted as $\{Enc_{K_i}(D_i)\}$
    \item The user gets $K_j$ from $\{K_i\}$ via $1$-out-of-$N$ OT protocol.
    \item The user gets encrypted $Enc_{K_j}(D_j)$ from $\{Enc_{K_i}(D_i)\}$ via PIR protocol.
    \item The user decrypts $Enc_{K_j}(D_j)$ with $K_j$.
\end{enumerate}
For the bandwidth overhead, the above scheme can achieve the same security with a bandwidth consumption of $\Psi(|D|+N*|K|)$. Given that $|D|\gg |K|$, the bandwidth overhead is $\Psi(|D|)$ which approximates the data downloaded size without any protection. For the performance overhead, the symmetric encryption phase can be conducted offline and thus can be omitted. The performance of PIR is highly optimized by using Ring-LWE \cite{xpir}. The overhead of decrypting $Enc_{K_j}(D_j)$ is negligible compared to the network latency. The overhead of bandwidth and performance is evaluated in Section \ref{sec:eval}.

